SNAP: Efficient Extraction of Private Properties with Poisoning

Property inference attacks allow an adversary to extract global properties of the training dataset from a machine learning model. Such attacks have privacy implications for data owners sharing their datasets to train machine learning models. Several existing approaches for property inference attacks against deep neural networks have been proposed, but they all rely on the attacker training a large number of shadow models, which induces a large computational overhead. In this paper, we consider the setting of property inference attacks in which the attacker can poison a subset of the training dataset and query the trained target model. Motivated by our theoretical analysis of model confidences under poisoning, we design an efficient property inference attack, SNAP, which obtains higher attack success and requires lower amounts of poisoning than the state-of-the-art poisoning-based property inference attack by Mahloujifar et al. For example, on the Census dataset, SNAP achieves 34% higher success rate than Mahloujifar et al. while being 56.5x faster. We also extend our attack to infer whether a certain property was present at all during training and estimate the exact proportion of a property of interest efficiently. We evaluate our attack on several properties of varying proportions from four datasets and demonstrate SNAP's generality and effectiveness. An open-source implementation of SNAP can be found at https://github.com/johnmath/snap-sp23.

==> Analysis.tex <==
\section{Effect of Poisoning on Logit Distribution}
\harsh{Please read Notations paragraph in section 3, before reading this.}

Let $\dist \equiv J(\rv{X},\rv{Y}) $ denote the original data distribution of clean samples.
%
We now describe the adversarial distribution $\dist_p$ introduced by the attacker.  To sample a data point from  $\dist_p$, the attacker first samples a data point $(x,y) \leftarrow \dist_f$, such that $f(x) = 1$ and $y = v$, where $v$ is the victim label. The attacker then chooses $\Tilde{v}$ as the truth label associated to this feature vector $x$. As result, the adversarial distribution can be viewed as $$\dist_p \equiv J(\rv{X}|(f(\rv{X}) = 1 \land \rv{Y} = \vlabel),~\tlabel)$$

For simplicity of explanation later in the proof, we replace `$\rv{X}|(f(\rv{X}) = 1 \land \rv{Y} = \vlabel)$' with $\rv{X^v_f}$. The above equation then becomes $\dist_p \equiv J(\rv{X^f_v},~\tlabel)$. 

%Let $\dist_p$ denote the distribution generated by the adversary such that when a data point is sampled from $\dist_p$, it has the target property $f(x) = 1$ with its original label as $\vlabel$, which is then adversarially changed to $\tlabel$.

After poisoning, the resulting distribution $\Tilde{\dist}$ can be viewed as a weighted mixture of $\dist$ and $\dist_p$, i.e. $$\Tilde{\dist}\equiv p.\dist_p + (1-p).\dist$$

Let $(\Tilde{\rv{X}},\Tilde{\rv{Y}})$ be the joint distribution of samples from $\Tilde{\dist}$. Let $t = \Pr[f(\rv{X}) = 1]$ and $\pi_v = \Pr[\rv{Y}=v | f(x)=1]$.  We now define two events:
\begin{itemize}
    \item[-] GE: Sampling a data point from $\dist$.
    \item[-] BE: Sampling a data point from $\dist_p$.
\end{itemize}

Consequently, if we sample a data point from $\Tilde{\dist}$, then with probability $p$, it could have been sampled from underlying distribution $\dist_p$, i.e. $\Pr[BE] = p$ and $\Pr[GE] = 1-p$ in this scenario. 
We now calculate the effect of poisoning on the  clean logit $\logitval{x}{\tlabel}$ with respect to target label $\tlabel$.

%
%from which also the training dataset gets sampled from, as 
% \begin{equation*}
%     \Tilde{\dist} \equiv
% \begin{cases}
%     \dist_p,& \text{with probability } p\\
%     \dist,              & \text{with probability } (1-p)
% \end{cases}
% \end{equation*}

%For simplicity we use  $\Pr[X_s = x]$ to denote $\Pr[X=x | f(x) = 1 \land Y = v]$.Let $(\Tilde{X},\Tilde{Y})$ be the joint distribution of samples from $\Tilde{\dist}$. 
%

%$PE$ and $GE$ be the events where the data point is sampled from $\dist_p$ and $\dist$ respectively. 

\begin{theorem}
For any $(x,y)$ sample, such that $f(x) = 1$ and $y = v$, the poisoned logit value with respect to target label $\tlabel$ can be written as
\begin{equation} \label{eqn:logit_eqn}
    \plogitval{x}{\tlabel} = \log{\left[\frac{p}{\pi_v(1-p)t} + e^{\logitval{x}{\tlabel}} \left( 1+\frac{p}{\pi_v(1-p)t}\right) \right]}
\end{equation}

\end{theorem}

\begin{proof}
We can write 
\begin{equation} \label{eqn:tgt_logit}
\plogitval{x}{\tlabel} = \log \left(\frac{\Pr[\Tilde{\rv{Y}} = \tlabel | \Tilde{\rv{X}} = x]}{1 - \Pr[\Tilde{\rv{Y}} = \tlabel | \Tilde{\rv{X}} = x]}\right) = \log\left(\frac{\Pr[\Tilde{\rv{Y}} = \tlabel | \Tilde{\rv{X}} = x]}{ \Pr[\Tilde{\rv{Y}} = \vlabel | \Tilde{\rv{X}} = x]}\right)
\end{equation}

We first calculate the probability $\Pr[\Tilde{\rv{Y}} = \vlabel | \Tilde{\rv{X}} = x]$. We can re-write this probability as 
\begin{multline*}
    \Pr[\Tilde{\rv{Y}} = \vlabel | \Tilde{\rv{X}} = x] = \Pr[\Tilde{\rv{Y}} = \vlabel |\Tilde{\rv{X}} = x \land GE].\Pr[GE| \Tilde{\rv{X}} = x] \\ + \Pr[\Tilde{\rv{Y}} = \vlabel | \Tilde{\rv{X}} = x \land BE].\Pr[BE|\Tilde{\rv{X}} = x]
\end{multline*}

Note that, when event $BE$ occurs $\Pr[\Tilde{Y} = \vlabel |\Tilde{X} = x \land BE] = 0$, as the sample when picked from $\dist_p \equiv J(\rv{X^f_v},~\tlabel)$, will have the associated label as $\tlabel$.  We can then re-write the above equation as 
\begin{equation} \label{eqn: v|x}
    \Pr[\Tilde{\rv{Y}} = \vlabel | \Tilde{\rv{X}} = x] = \Pr[\Tilde{\rv{Y}} = \vlabel |\Tilde{\rv{X}} = x \land GE].\Pr[GE|\Tilde{\rv{X}} = x]
\end{equation}

\smallskip
We now calculate  $\Pr[GE|\Tilde{X} = x]$ using Bayes' theorem as follows:
\begin{multline} \label{eqn:GE|X}
    \Pr[GE|\Tilde{\rv{X}} = x] = \frac{\Pr[\Tilde{\rv{X}} = x | GE].\Pr[GE]}{\Pr[\Tilde{\rv{X}} = x | GE].\Pr[GE] + \Pr[\Tilde{\rv{X}} = x | BE].\Pr[BE]}
    \\ = \frac{\Pr[\Tilde{\rv{X}} = x | GE].(1-p)}{\Pr[\Tilde{\rv{X}} = x | GE](1-p) + \Pr[\rv{X^v_f} = x].p}
\end{multline}

Note that, probability $\Pr[\Tilde{\rv{X}} = x | GE] = \Pr[\rv{X} = x]$.
We can then re-write probability $\Pr[\rv{X} = x]$ as follows:
\begin{flalign*}
    \Pr[\rv{X} = x] = \Pr[\rv{X} = x|\rv{Y}=\vlabel \land f(x) = 1 ].\Pr[\rv{Y}=\vlabel \land f(x) = 1] \\+ \Pr[\rv{X} = x|\overline{\rv{Y}=\vlabel \land f(x) = 1} ].\Pr[\overline{\rv{Y}=\vlabel \land f(x) = 1}]
\end{flalign*}

However, $\Pr[\rv{X} = x|\overline{Y=\vlabel \land f(x) = 1} ] = 0$ as we only consider $(x,y)$ samples such that $f(x)=1$ and $y=v$. We can then simplify the above equation as follows:

\begin{flalign*}
\Pr[\rv{X} = x]= \Pr[\rv{X} = x|\rv{Y}=\vlabel \land f(x) = 1 ].\Pr[\rv{Y}=\vlabel \land f(x) = 1]
\\=\Pr[\rv{X}=x| \rv{Y}=\vlabel \land f(x) = 1 ]. \Pr[\rv{Y}=\vlabel| f(x)=1]. \Pr[f(x)=1] 
\\= \Pr[\rv{X^v_f} = x].\pi_v.t
\end{flalign*}
Now substituting the above equation in Eqn.\ref{eqn:GE|X}, we get:

\begin{multline*}
    \Pr[GE|\Tilde{\rv{X}} = x] = \frac{\Pr[\rv{X^v_f} = x].\pi_v.t.(1-p)}{\Pr[\rv{X^v_f} = x].\pi_v.t.(1-p) + \Pr[\rv{X^v_f} = x].p}
    \\= \frac{\pi_v (1-p)t}{\pi_v (1-p)t+p}
    % = \frac{\pi_v (1-p)t}{p+\pi_v (1-p)t}
\end{multline*}

And finally substituting the above in Eqn.\ref{eqn: v|x}, we get:
\begin{equation} \label{eqn:v|xintermsofpt}
    \Pr[\Tilde{\rv{Y}} = \vlabel | \Tilde{\rv{X}} = x] =  \frac{\pi_v (1-p)t}{p+\pi_v (1-p)t} . \Pr[\rv{Y} = \vlabel | \rv{X} = x]
\end{equation}

Similarly, we can calculate probability  $\Pr[\Tilde{\rv{Y}} = \tlabel | \Tilde{\rv{X}} = x]$ using Eqn.\ref{eqn:v|xintermsofpt} as follows
\begin{multline} \label{eqn:t|xintermsofpt}
    \Pr[\Tilde{\rv{Y}} = \tlabel | \Tilde{\rv{X}} = x] = 1 - \Pr[\Tilde{\rv{Y}} = \vlabel | \Tilde{\rv{X}} = x] 
    \\= 1 - \frac{\pi_v (1-p)t}{p+\pi_v (1-p)t} . \Pr[\rv{Y} = \vlabel | \rv{X} = x]
    \\= \frac{p}{p+\pi_v(1-p)t} + \frac{\pi_v(1-p)t}{p+\pi_v(1-p)t} \Pr[\rv{Y} = \tlabel | \rv{X} = x]   
\end{multline}

Substituting Eqn.\ref{eqn:v|xintermsofpt} and Eqn.\ref{eqn:t|xintermsofpt} back into Eqn.\ref{eqn:tgt_logit} and simplifying the equation, we get:
\begin{equation*}
    \plogitval{x}{\tlabel} = \log{\left[\frac{p}{\pi_v(1-p)t} + e^{\logitval{x}{\tlabel}} \left( 1+\frac{p}{\pi_v(1-p)t}\right) \right]}
\end{equation*}
\end{proof}
 
We now analyze the behavior of random variable $\plogitval{x}{\tlabel}$ under certain assumptions.

\begin{theorem}
Given logit value $\logitval{x}{\tlabel} \sim N(\mu, \sigma^2)$ follows a Gaussian distribution and the corresponding poisoned logit $\plogitval{x}{\tlabel}$ also follows a Gaussian distribution. The mean and variance of $\plogitval{x}{\tlabel}$ are $ \Tilde{u} = {\log{M} - \log{\left(\sqrt{\frac{V}{M^2}+1}\right)}}$ and $\Tilde{\sigma}^2 = \log{\left( \frac{V}{M^2} + 1\right)}$ respectively, where $M$ and $V$ denote the mean and variance of log-normal random variable $e^{\plogitval{x}{\tlabel}}$.
\end{theorem}

\begin{proof}
We re-write Eqn.\ref{eqn:logit_eqn} as follows:
\begin{equation*}
    e^{\plogitval{x}{\tlabel}} = \frac{p}{\pi_v(1-p)t} + e^{\logitval{x}{\tlabel}} \left( 1+\frac{p}{\pi_v(1-p)t}\right)
\end{equation*}
Under the assumption that logit value $\logitval{x}{\tlabel}$ is a Gaussian random variable,  random variable $e^{\logitval{x}{\tlabel}}$ as a consequence follows log-normal distribution with mean $e^{~\mu + \sigma^2/2}$ and variance $(e^{\sigma^2} -1).(e^{~2\mu + \sigma^2})$. We now compute the mean of the random variable $e^{\plogitval{x}{\tlabel}}$ as follows:

\begin{multline}
  M = \mathbb{E}[e^{\plogitval{x}{\tlabel}}] = \mathbb{E}\left[ \frac{p}{\pi_v(1-p)t}+ e^{\logitval{x}{\tlabel}} \left( 1+\frac{p}{\pi_v(1-p)t}\right) \right]
  \\=  \frac{p}{\pi_v(1-p)t} + \mathbb{E}[e^{\logitval{x}{\tlabel}}] . \left( 1+\frac{p}{\pi_v(1-p)t}\right)
  \\= \frac{p}{\pi_v(1-p)t} + e^{~\mu + \sigma^2/2} .  \left( 1+\frac{p}{\pi_v(1-p)t}\right)
\end{multline}

Similarly, we compute the variance of $e^{\plogitval{x}{\tlabel}}$ as

\begin{multline}
    V = \mathbf{Var}(e^{\plogitval{x}{\tlabel}}) = \mathbf{Var}\left(\frac{p}{\pi_v(1-p)t}+ e^{\logitval{x}{\tlabel}} \left( 1+\frac{p}{\pi_v(1-p)t}\right) \right)
    \\= \mathbf{Var}(e^{\logitval{x}{\tlabel}}).\left( 1+\frac{p}{\pi_v(1-p)t}\right)^2
    \\= (e^{\sigma^2} -1).(e^{~2\mu + \sigma^2}).\left( 1+\frac{p}{\pi_v(1-p)t}\right)^2
\end{multline}

Note that, based on Eqn.\ref{eqn:logit_eqn}, when the term $\frac{p}{\pi_v(1-p)t}>0$ then the random variable $\plogitval{x}{\tlabel}$ does not follow a Gaussian distribution naturally. However, for simplicity of analysis we approximate its distribution to be Gaussian with $\Tilde{u}$ and $\Tilde{\sigma}^2$ denoting its mean and variance respectively. As a result random variable $e^{\plogitval{x}{\tlabel}}$ follows a log-normal distribution with mean and variance as $M$ and $V$ respectively. We can now write a system of equations as: $e^{\Tilde{u} + \Tilde{\sigma}^2/2} = M$ and $(e^{\Tilde{\sigma}^2-1}).(e^{2\Tilde{\mu} + \Tilde{\sigma}^2}) = V$. On solving for $\Tilde{u}$ and $\Tilde{\sigma}^2$, we get:  
\begin{flalign*}
    \Tilde{u} = {\log{M} - \log{\left(\sqrt{\frac{V}{M^2}+1}\right)}}
    \\  \Tilde{\sigma}^2 = \log{\left( \frac{V}{M^2} + 1\right)}
\end{flalign*}

\end{proof}

\begin{figure}[h]{
%		\centering
		\begin{subfigure}[b]{0.5\textwidth}
			
			\includegraphics[width=0.5\textwidth]{Theoretical_Plots/Mean-Black-Census.pdf}%
			\includegraphics[width=0.5\textwidth]{Theoretical_Plots/Mean-WhiteMale-Adult.pdf}%
			
			\caption{\footnotesize Mean of logits as a function of poisoning fraction.}
			\label{sfig:mean}
		\end{subfigure}
	%
		\begin{subfigure}[b]{0.5\textwidth}
			\includegraphics[width=0.5\textwidth]{Theoretical_Plots/Variance-Black-Census.pdf}%
			\includegraphics[width=0.5\textwidth]{Theoretical_Plots/Variance-WhiteMale-Adult.pdf}%
			\caption{ \footnotesize Variance of logits as a function of poisoning fraction.}
			\label{sfig:var}
		\end{subfigure}
		%
	\caption{Theoretical and Experimental plots on the behavior of logits depending on the poisoning amount}
	\label{fig:TheoreticalandExperimentalResults}
}
\end{figure}

==> Attack_Analysis.tex <==


\section{Attack Analysis}
\subsection{ Threshold Computation} \label{sec:thresholdcomp}
\matthew{I believe this is a consequence of the Neyman Pearson Lemma}

\alina{Remove this and just mention we pick threshold that minimizes the error.}

\harsh{I see, is the below part very trivial?}



\begin{proposition}
Given  two Gaussian distributions $X_0 \sim N(\mu_0,\sigma_0)$ and $X_1\sim N(\mu_1,\sigma_1)$  and an objective function $ J = \pt{0}+\pt{1}$, where $\pt{0} = \Pr[X_0>\threshold]$ and $ \pt{1} = \Pr[X_1<\threshold]$, the  threshold $\threshold$ that  minimizes $J$ is ...  
\end{proposition} \label{thm:thresholdcomp}

%\harsh{By mistake I solved it for the reverse case, need to switch  $\world{0}$ with $\world{1}$ and vice versa everywhere, otherwise the proof follows. Do recheck the proof below}
\begin{proof}
Our goal is to find threshold $\threshold$ that minimizes the objective function $J =  \pt{0}+\pt{1}$. We re-write the objective function as follows:
\begin{align*}
	J = \pt{1}+\pt{0} =   \Pr[X_0> \threshold] + \Pr[X_1<\threshold] 
	\\= \Pr[X_1<\threshold] + 1 - \Pr[X_0<\threshold] 
	\\= 1 + \Phi\left(\frac{\threshold-\mu_1}{\sigma_1}\right) - \Phi\left(\frac{\threshold-\mu_0}{\sigma_0}\right)
\end{align*}

where $\Phi\left(\frac{\threshold-\mu_i}{\sigma_i}\right)$ denotes the CDF of the random variable $X_i$. To compute the optimal value of $\threshold$, we differentiate $J$ with respect to  $\threshold$ and solve the equation is as follows:

\begin{align*}
	\frac{\partial J}{\partial \threshold} = \frac{\partial }{\partial \threshold}  \Phi\left(\frac{\threshold-\mu_1}{\sigma_1}\right) -  \frac{\partial}{\partial \threshold}  \Phi\left(\frac{\threshold-\mu_0}{\sigma_0}\right)  
	\\=  \frac{1}{\sigma_1}\phi\left(\frac{\threshold-\mu_1}{\sigma_1}\right) - \frac{1}{\sigma_0}\phi\left(\frac{\threshold-\mu_0}{\sigma_0}\right)
\end{align*}
where $\phi\left(\frac{\threshold-\mu_i}{\sigma_i}\right)$ denotes the PDF of the random variable $X_i$. Setting  the above equation to $0$ and substituting the gaussian PDF equation for $\phi$, we get:

\begin{equation*}
	%\frac{1}{\sigma_{\world{0}}}\phi\left(\frac{\threshold-\mu_{\world{0}}}{\sigma_{\world{0}}}\right)  = \frac{1}{\sigma_{\world{1}}}\phi\left(\frac{\threshold-\mu_{\world{1}}}{\sigma_{\world{1}}}\right) 	
	e^{{-(\threshold-\mu_1)^2}/{2\sigma_1^2}}  = \left({\sigma_1}/{\sigma_0}\right)^2  e^{{-(\threshold-\mu_0)^2}/{2\sigma_0^2}} 
\end{equation*}

On re-arranging the above equation:
\begin{equation} \label{eq:logit_val}
%	\sigma_{\world{0}}^2{(\threshold-\mu_{\world{1}})^2} - \sigma_{\world{1}}^2{(\threshold-\mu_{\world{0}})^2} = 4\sigma_{\world{0}}^2\sigma_{\world{1}}^2\log\left(\frac{\sigma_{\world{0}}}{\sigma_{\world{1}}}\right)	
\footnotesize
(\sigma_1^2 - \sigma_0^2)\threshold^2 + 2(\mu_1\sigma_0^2 - \mu_0\sigma_1^2) \threshold + \mu_0^2\sigma_1^2 -\mu_1^2\sigma_0^2 
+ 4\sigma_1^2\sigma_0^2\log\left({\sigma_0}/{\sigma_1}\right) = 0
\end{equation}
The roots of equation \ref{eq:logit_val} can then be written as:
\begin{equation*}
	\small
	T = \frac{(\mu_0\sigma_1^2 - \mu_1\sigma_0^2) 
			\pm 2\sigma_1 \sigma_0 \sqrt{\left(\frac{\mu_1-\mu_0}{2}\right)^2 
				+(\sigma_0^2 - \sigma_1^2) \log \left(\frac{\sigma_0}{\sigma_1}\right) }}
		{\sigma_1^2 - \sigma_0^2}
\end{equation*}
\end{proof}  

An interesting observation is when the standard deviations for the two Gaussians are the same, i.e. $\sigma_0 = \sigma_1$. Revisiting equation \ref{eq:logit_val} with the above condition gives us:
\begin{align*}
	 \threshold = \frac{ \mu_1^2\sigma_1^2 -\mu_0^2\sigma_1^2} {2(\mu_1\sigma_1^2 - \mu_0\sigma_1^2)} 
\end{align*}
 
 After simplifying the above equation, we get the value of logit threshold as $T = (\mu_0+ \mu_1)/2$. Thus, if the standard deviations of the two Gaussians are very close to each other then $T = (\mu_0+ \mu_1 )/2$ is a good estimate.
%Once the poisoned dataset $D_p$ is constructed, it is used as a part of the training dataset  to train the black-box model $\mathcal{M}_p$. Algorithm \ref{alg:blackbox} provides the  steps for the $(t_0,t_1)$-distinguishing test followed by the adversary. 

%Next, we talk about how to build our distinguishing test.


\subsection{Number of Test Queries} 
\label{sec:num_queries}

In this section, we discuss the number of test samples required by the adversary to succeed  distinguishing the two worlds as described in algorithm \ref{alg:adv_steps}.

\begin{proposition} \label{thm:num_queries}
	Given  non-ideal probabilities $\pt{0}$ and $\pt{1}$, the number of queries $q$ required by the adversary $\Adv$ to succeed the distinguishing test with  probability at least $1-c$ is $ q = \underset{i\in\{0,1\}}{\mathrm{max}}\, \frac{-(2+\delta_i) \log c }{\delta_i^2 \pt{i}}$ , where $\delta_i =  \frac{1}{2\pt{i}}-1$.
\end{proposition} 

\begin{proof}
	%Without loss of generality, assume we are in the $t_1$ world.  
	We  define a Bernoulli random variable as follows
	\begin{align*}
		b = 
		\begin{cases}
			1, & \text{w.p.}~\pt{1}= \Pr[\ w< \threshold] \\
			0, & \text{otherwise}
		\end{cases}
	\end{align*}
	where $w= \log({\hat{y}}/{1-\hat{y}})$   from Algorithm \ref{alg:blackbox}. Suppose we predict $\world{1}$ world if and only if $\Pr[(X_1 = \sum_{i=1}^{q_1} b_{i})  > q_1/2] < c$, for some very small probability $c$. 
	
	We can then bound this probability by applying Chernoff bound, with $\delta>0$, as follows:
	\begin{align*}
		\Pr[X_1 > \frac{q}{2}] = \Pr[X_1 > (1+ \delta)\mu] < e^{\frac{-\delta^2 \mu}{2+\delta}}
	\end{align*}
	where $\mu = q_0\pt{0}$ is the mean of $X_1$ and $\delta = \frac{1}{2\pt{1}}-1$. Condition $\delta>0$ implies $\pt{1}<1/2$. Now solving for $ e^{\frac{-\delta^2 \mu}{2+\delta}} = c$, we get $$q_1 = \frac{-(2+\delta) \log c }{\delta^2 \pt{1}}$$
	
	Similarly, we define a Bernoulli random variable, for the $\world{0}$ world,  as follows:
	\begin{align*}
		b' = 
		\begin{cases}
			1, & \text{w.p.}~\pt{0}= \Pr[\ w> \threshold] \\
			0, & \text{otherwise}
		\end{cases}
	\end{align*} 
	We predict $\world{0}$ world if and only if $\Pr[(X_0 = \sum_{i=1}^{q_1} b'_{i})  > q_1/2] < c$. On applying Chernoff bound and solving for $q_0$, we get
	
	$$q_0= \frac{-(2+\delta) \log c }{\delta^2 \pt{0}}$$
	where $\delta = \frac{1}{2\pt{0}}-1$ and $\pt{0} < 1/2$.  We then set the number of queries $q = \text{max}(q_0, q_1)$. 
	
\end{proof}
To interpret Theorem \ref*{thm:num_queries}, we plot  Figure \ref{fig:QueryPlot}  which shows the number of queries  required as a function of success probability $(1-c)$ and non-ideal probabilities $\pt{0}$ and $\pt{1}$. We observe that for smaller values of non-ideal probabilities  the total number of queries required to distinguish the two worlds, with high confidence, is very small. For instance, for $p_t = 0.2$, we require less than $50$ queries to distinguish the two worlds with probability of success $1-c$ set to $0.999$. Even for higher values of 
$p_t$ such as $p_t= 0.4$, we require no more than $650$ queries to distinguish the two worlds with success probability of $0.999$.

\begin{figure}[h]
	\centerline{%
		\includegraphics[width=0.5\textwidth]{QueriesPlot}%
	}%
	\caption{Number of queries as a function of success probability  and maximum of  the non-ideal probabilities $p = \text{max}(\pt{0},\pt{1})$ }
	\label{fig:QueryPlot}
\end{figure}


\begin{comment}
\subsection{Choosing number of poisoning samples} 
\harsh{I don't think we need this anymore. We can now replace it with effect of poisoning on Logit Distribution.}
\label{sec:paramk}
Given $t_0$ and $t_1$ fraction of  samples with target property $f$ in the training set, the choice of $k$ plays a crucial role in the behavoir of the logits in both worlds.  We provide a formal analysis on the choice of $k$ as a function of $\mt{0}$ and $\mt{1}$ and also discuss the necessary inequality conditions that arise in our analysis between the three parameters.

%{\it Choice of k:} 

\begin{lemma} \label{lem:as1}
	Given a subpopulation $\subtgt$ of size $n$, with $X \sim \dist_f$ and class label $v$. If we add k poisoning examples from same distribution $X_p \sim \dist_f$ and class label $v'$, the probability that the Bayes optimal classifier makes prediction $v$ for a sample $x \in \subtgt$ is $n/n+k$.
\end{lemma}

\begin{proof}
	Given  $n$ samples in target subpopulation $\subtgt$ with victim label $v$ and $k$ poisoned samples injected in $\subtgt$  with target label $\tilde{v}$ ,  the probability of predicting $v$  given a sample $x \in \subtgt$ can be written as:
	\begin{align*}
		&\Pr[Y = v| X=x]  = \frac{\Pr[X=x| Y=v].\Pr[Y=v]}{\Pr[X=x]}
		\\&= \frac{\Pr[X=x| Y=v].\Pr[Y=v]}{\Pr[X=x| Y=v].\Pr[Y=v] + \Pr[X=x| Y=\tilde{v}].\Pr[Y=\tilde{v}]}
	\end{align*}
\end{proof}

We denote $\rho_i(x)  = \Pr[X=x| Y=i]$ and $\pi_i = \Pr[Y=i]$, where $i \in \{v,\tilde{v}\}$. Note that $\pi_v + \pi_{\tilde{v}}  = 1$ as all the samples in $S_f$ will   either have class label $v$ or $\tilde{v}$ (introduced due to poisoning). The adversary can estimate  $\pi_i$  by  counting the fraction  of occurrences of class label $i$ in the target subpopulation. We denote the estimated value  as $\hat{\pi}_i$. We can then re-write the above equation as follows:

\begin{align*}
	&\Pr[Y = v| X=x] = \frac{\rho_v(x).\hat{\pi}_v}{\rho_v(x).\hat{\pi}_v +\rho_{\tilde{v}}(x).\hat{\pi}_{\tilde{v}}}
\end{align*}
Recall that,  adversary injects $k$ poisoned samples which were originally part of $S_f$ but have their class label changed to $\tilde{v}$. As a consequence, both $\rho_v$ and $\rho_{\tilde{v}}$ will follow a very similar distribution. We can then simplify the above equation as follows:

\begin{align*}
	&\Pr[Y = v| X=x] = \frac{\hat{\pi}_{{v}}}{\hat{\pi}_{{v}} + \hat{\pi}_{\tilde{v}} } = \frac{\frac{n}{k+n}}{\frac{n}{k+n} + \frac{k}{k+n}} = \frac{n}{n+k}
\end{align*}


%\begin{theorem} \label{thm: param_estimates}
	
	%Given  $\mt{0}$ samples with target property $f$ in $\world{0}$ world, the number of poisoned samples required to be injected in the target subpopulation $\subtgt$ such that  the model trained  in $t_0$ world behaves worse than a random classifier  for  samples in $\subtgt$, is $k = (1+\delta_\world{0})\alpha_vm_{\world{0}}$, where $\delta_\world{0} = \frac{-\log c + \sqrt{\log^2 c - 8 ~\alpha_vm_{\world{0}} \log c}}{2\alpha_vm_{\world{0}} }$ and $\alpha_{v}$ is the fraction of samples with victim class `$v$' among the samples exhibiting $f$. Consequently, the minimum number of samples $\mt{1}$ required  for the model trained in $\world{1}$ world to perform better than a random classifier is $ \mt{1} = (1+ \delta_{\world{0}})\beta\mt{0} - \frac{\log c} {\alpha_v}  + \sqrt{\frac{\log^2 c} {\alpha^2_v}  - 2 (1+ \delta_\world{0})\beta \mt{0}\frac{\log c} {\alpha_v} }$ \harsh{Unfortunately the theorem statement reads like a paragraph but gives the general idea. Need to condense the theorem statement}
%\end{theorem} 

\begin{proposition}
	Given $\mt{0}$ samples with target property $f$, 
	\begin{itemize}
		\item[--] If the number of poisoned samples $k \geq (1+\delta_0)\alpha_vm_0$,  then the probability of predicting the incorrect class for a sample $x \in S_f$ is greater than $1/2$, where $\delta_0 = \frac{-\log c + \sqrt{\log^2 c - 8 ~\alpha_vm_0 \log c}}{2\alpha_vm_0 }$ and $\alpha_{v}$ is the fraction of samples with victim class `$v$' among all samples that have property $f$ .
		
		\item[--] If the number of samples $ \mt{1} \geq (1+ \delta_0)\mt{0} - \frac{\log c} {\alpha_v}  + \sqrt{\frac{\log^2 c} {\alpha^2_v}  - 2 (1+ \delta_0) \mt{0}\frac{\log c} {\alpha_v} }$ with target property $f$ are present in $\world{1}$ world, then the probability of predicting the incorrect class for a sample $x \in S_f$ is less than $1/2$.
	\end{itemize}
	
\end{proposition}

\begin{proof}
	Recall the adversary has access to $\mathcal{D}_f$. The adversary uses knowledge of $\mathcal{D}_f$  to  estimate  the fraction of  victim class $\alpha_{v}$ among all samples with target property $f$ as follows: sample $m'>0$ instances from $\mathcal{D}_f$ and compute $\alpha_{v} = {\sum_{i=1}^{m'}\mathbbm{1}\{y_i = v\} }/{m'}$. 
	\harsh{Justification: We can use  confidence intervals such as Clopper-Pearson to give  a bound on true $\alpha$ being in a close range of the estimated  $\alpha_{v}$ with very high probability, given enough samples.}
	
	The number of samples  in  subpopulation $\subtgt$ can be  viewed as a binomial distribution $ Bin(\mt{0}, \alpha_v)$, i.e. $X_{0} = \sum_{i=1}^{\mt{0}} \text{Bernoulli}(\alpha_v)$.  We can then use the following multiplicative Chernoff bound, with $\delta>0$:
	$$\Pr[X_{0}>(1+\delta)\mu]  < e^{\frac{-\delta^2 \mu}{2 + \delta}} = c$$
	
	
	Setting the mean $\mu = \alpha_v \mt{0}$  and solving $e^{\frac{-\delta^2 \mu}{2 + \delta}} = c$, we get a quadratic equation in $\delta$ as follows:
	
	$$\alpha_v\mt{0} \delta^2 + \log c ~\delta + 2\log c = 0$$
	The root of the equation always satisfying $\delta>0$ is $$\delta_0 = \frac{-\log c + \sqrt{\log^2 c - 8 ~\alpha_v\mt{0} \log c}}{2\alpha_v\mt{0} }$$
	
	
	%Setting the mean $\mu = \alpha_v m_{\world{0}}$ and $\delta = 1$ in the above Chernoff bound, we get:
	%$$\Pr[X_{\world{0}}>2\alpha_v  \mt{0}] < e^{\frac{-\alpha_v \mt{0}}{3}}$$
	
	The bound tells us that the number of samples in $\subtgt$ is less than $(1+\delta_0)\alpha_v\mt{0}$ with probability at least $1- c$. As a result, the adversary can set  the number of poisoned samples $k = (1+\delta_0)\alpha_v\mt{0}$ in Algorithm \ref*{alg:prop_poison}. Setting $n  = (1+\delta_0)\alpha_v\mt{0}$ and $k \geq m'$ in Lemma \ref{lem:as1}, we get: 
  
  \begin{align*}
  	&\Pr[Y = v| X=x] =  \frac{n}{n+k} \leq \frac{n}{n+n} = \frac{1}{2}.
  \end{align*}

As a consequence, the probability of predicting the incorrect label for a sample $x \in \subtgt$ becomes $\geq 1/2 $.
	
	%The bound tells us that the number samples belonging to  the victim class is less than $2\alpha_v \mt{0}$ with probability atleast $1- e^{-\alpha_v \mt{0}/3}$.  As a result, the adversary can set  the number of poisoned samples $k = 2\alpha_v \mt{0}$ in Alogorithm \ref*{alg:prop_poison}.
	
	We now analyze the $t_1$ world and the number of samples $\mt{1}$ the adversary should ideally choose. 
	 %For simplicity of our proof we assume $\alpha^{\world{0}}_{v}  = \alpha^{\world{1}}_{v} = \alpha_v$. Note that, this is a soft assumption as ideally one would want these estimates to be  as close to the true mixture coefficient as possible.  
	The number of samples in $\subtgt$ for this case is $X_1 = \sum_{i=1}^{\mt{1}} \text{Bernoulli}(\alpha_v)$. Note that we would ideally want $X_1$ to be substantially greater than $k$, so that the influence of poisoning is minimal. As a result, we make  $X_1$  to be at least $\beta > 1$ times the size of $k$ with very high probability, where $k = (1+\delta_0)\alpha_v\mt{0}$.  Applying  multiplicative Chernoff  bound, with $0 \leq \delta \leq 1$:
	
	$$\Pr[X_1\leq(1-\delta)\mu]  \leq e^{\frac{-\delta^2 \mu}{2}} $$
	
	The mean  in this case is $\mu = \alpha_v \mt{1}$. Note that, we want $(1-\delta)\mu$ to be equal to $\beta k$. On solving for $\delta$, we get:
	
	$$\delta = 1 - \frac{\beta k}{\alpha_v\mt{1}} = 1 - \frac{(1+\delta_0) \beta\mt{0}}{\mt{1}}$$
	
	Condition $0 \leq \delta \leq 1$ also implies $\mt{1} \geq (1+\delta_0) \mt{0}$. As a result, the above Chernoff bound equation can be written as:
	\begin{align*}
		\Pr[X_1 \leq \beta k]  \leq  e^{\frac{-\delta^2 \mu}{2}}
		%\Pr[X_{\world{1}} \leq \beta k]  \leq  e^{\frac{-(1-\frac{4\mt{0}}{\mt{1}})^2 \alpha_v \mt{1}}{2}} 
		% \\= \Pr[X_{\world{1}} \leq \beta k]  \leq  e^{\frac{-\alpha_v (\mt{1}-4\mt{0})^2 }{2\mt{1}}}
	\end{align*}
	
	On solving for $e^{\frac{-\delta^2 \mu}{2}} = c$ and substituting $\delta = 1 - {(1+\delta_0) \beta\mt{0}}/{\mt{1}}$, we get a quadratic equation in $\mt{1}$ as follows:
	$$\mt{1}^2 - 2 ((1+\delta_0)\beta\mt{0} -\frac{\log c} {\alpha_v} ) \mt{1} + (1 + \delta_0)^2 \beta^2\mt{0}^2 = 0$$
	
	The root  satisfying the above equation and the constraint $\mt{1} \geq (1+\delta_0)\beta \mt{0}$ is
	\begin{equation*}
\footnotesize 
\mt{1} = (1+ \delta_0)\beta\mt{0} - \frac{\log c} {\alpha_v}  + \sqrt{\frac{\log^2 c} {\alpha^2_v}  - 2 (1+ \delta_0)\beta \mt{0}\frac{\log c} {\alpha_v} }
	\end{equation*}

	The bound tells us that when we set the number of samples $\mt{1}$ with target property $f$ as the above value, then the number of samples in $\subtgt$ is greater than $\beta k$ with probability atleast $1-c$. So if we set $\beta =1$,  $n  \geq \beta k$  in Lemma \ref{lem:as1}, we get: 
	
	\begin{align*}
		&\Pr[Y = v| X=x] =  \frac{n}{n+k} \geq \frac{n}{n+n} = \frac{1}{2}.
	\end{align*}
	
	As a consequence, the probability of predicting the incorrect label for a sample $x \in \subtgt$ remains $\leq  1/2$.
	
\end{proof}

\harsh{Suggestion: We can also probably add a para to explain the above theorem by  setting different values for $\beta$, $c$, $\mt{0}$, $\mt{1}$ to show the probability of making  an error using lemma \ref{lem:as1}}
\end{comment}


==> Conclusion.tex <==
\section{Conclusion}

We introduce an efficient property inference attack motivated by sound theoretical analysis of the effects of poisoning on model confidence distributions. Our distinguishing test attack, \system, outperforms prior work \cite{Ganju18, Chase21, DistributionInference} in multiple settings while requiring several orders of magnitude fewer shadow models. This resulted in a $50.8 \times$ speed increase on CPU when compared to \cite{Chase21} in our testing. Our attack is more effective at lower poisoning rates than \cite{Chase21}. 


% We are able to achieve attack success above 90\% with 8 poisoned samples on small properties, 1\% poisoning on medium properties, and 3.5\% poisoning on large properties. 
%Additionally, prior work does not include results for property inference on small properties. \system\ is able to perform distinguishing tests on a wide variety of properties while remaining imperceptible and having a minimal impact on the utility of the target model.

We also introduce extensions and optimizations to \system. By using the optimized poisoning method, we are able to have a more imperceptible attack with lower poisoning rate, while increasing the success of our distinguishing test. Our property existence attack extends \system\ to be a generalization of membership inference, where we are able to determine if a group of individuals with a certain property have been used in training the target model. The property size estimation attack generalizes \system\ by requiring no prior knowledge of possible fractions $t_{0}$ and $t_{1}$. Our property size estimation attack is also able to make precise estimates with low poisoning rates, while requiring logarithmically fewer shadow models than \cite{DistributionInference} and \cite{Chase21}.


==> alternate_theorem_b1.tex <==
\section{Effect of Poisoning on the Predicted Logit Distribution (Revised)}

Let the original set of clean samples be $\dist_{C} = (X,Y)$ where $(X, Y)$ is defined as an enumerable collection of ordered pairs of data points, $x_{i}$ and their corresponding original labels $y_{i}$. Formally, $\dist_{C} = \{(x_{1}, y_{1}), \dots \}$. We will also define a bit $b_{i}$ that denotes whether a given sample $(x_{i}, y_{i})$ was poisoned.
Let $\dist_{P}$ be the set of poisoned samples. For all samples, $(x_{j}, \tilde{y}_{j}) \in \dist_{P}$, $b_{i} = 1$, which tells us that the original label $y_{j} = v$ has been adversarially flipped so that each sample in $\dist_{P}$ is $(x_{i}, \tilde{v})$. \harsh{I think we should also mention each such $x_i$ in $\dist_{P}$ has property $f(x_i)=1$} Additionally, for every data point, $x_{i}$, we define a bit that denotes whether $x_{i}$ has the target property. We will say $f(x_{i}) = 1$ if $x_{i}$ has the  the target property; otherwise, $0$. The dataset that we will sample our training set from can be written as the union of the clean set and the poisoned set

\begin{align*}
    \Tilde{\dist} &= \dist_{C} \cup \dist_{P} = (\tilde{X}, \tilde{Y}) \\
    &= \{ x_{1}, y_{1}, \dots x_{k + 1}, \tilde{y}_{k + 1} \dots \} \: \text{, where $k = \vert \dist_{C} \vert$}
\end{align*}

When we sample uniformly from $\tilde{\dist}$ we receive an integer index, $i$, and its associated sample $(x_{i}, y_{i}) \in \tilde{\dist}$. We denote the probability that we sample from $\tilde{\dist}$ and get a sample that is also in $\dist_{C}$ as $\mathbb{P}_{i \sim \tilde{D}}[b_{i} = 0] = 1 - p$. Similarly, we will define the probability of picking a sample that comes from $\dist_{P}$ as $\mathbb{P}_{i \sim \tilde{D}}[b_{i} = 1] = p$. 

 We will define the probability of drawing a sample, $(x, y)$ uniformly over each dataset with $f(x)  = 1$ as the following. $\mathbb{P}_{\dist_{C}}[f(x) = 1] = t$,  $\mathbb{P}_{\dist_{P}}[f(x) = 1] = 1$, and   $\mathbb{P}_{\tilde{\dist}}[f(x) = 1] = t \cdot (1 - p) + p$. One should note, $\forall (x, y) \in \dist_{P}$, $x$ has the target property and original label $y = v$, which is flipped to $\tilde{v}$ during poisoning.

Lastly, we will define our clean logit (with respect to some label $\ell$) as a randomized prediction $\phi_{\ell}: X \rightarrow \mathbb{R}$. 
Given a sample $(x, y)$, we denote the probability of predicting the label $v$ when $f(x) = 1$ as $\mathbb{P}_{\phi}[\hat{Y} = v \vert f(x) = 1] = \pi_{v}$ (i.e., $\forall x, \: $ such that $f(x) = 1, \: \mathbb{P}_{\phi}[\hat{Y} = v |x \wedge f(x) = 1] = \pi_{v}$).
Now, we can compute the effect of poisoning on the clean logit value $\phi(x)_{\tilde{v}}$ with respect to the target label $\tilde{v}$
{\color{blue}We need to talk about probability for a fixed person in the dataset getting different labels, dependent on the classifier (i.e. consider the randomness of the classifier) - Jon}


% Theorem B.1.

\harsh{The poisoned logit seems to be defined as a function of not just the original logit but also $\pi_v$, which seems to be dependent on $\hat{Y}$ which in turn is a function of $\tilde{D}$}

\begin{theorem}
For all $(x, y) \in \tilde{\dist}$ with original label, $y = v$, and target property $f(x) = 1$, the poisoned logit value with respect to the target label, $\tlabel$, can be written as
\begin{equation} \label{eqn:logit_eqn}
\plogitval{x}{\tlabel} = \log \Bigg( e^{\phi(x)_{\tlabel}}  + \frac{1}{\pi_v} \Big( \frac{t \cdot (1-p + p)}{t \cdot (1 - p)} - 1 \Big) \Bigg)
\end{equation}
\end{theorem}


\begin{proof}
We can write the poisoned logit value as the following 
\begin{equation} \label{eqn:tgt_logit}
    \plogitval{x}{\tlabel} = \log \Big( \frac{\mathbb{P}_{\tilde{\phi}}[\hat{Y} = \tlabel \vert \: x]}{1 - \mathbb{P}_{\tilde{\phi}}[\hat{Y} = \tlabel \vert \: x]} \Big) = 
    \log \Big( \frac{\mathbb{P}_{\tilde{\phi}}[\hat{Y} = \tlabel \vert \: x]}{ \mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \: x]} \Big)
\end{equation}

First, we will compute the denominator, $\mathbb{P}[\hat{Y} = v \vert \: x]$. Using the law of total probability and $b$ to denote $(x, y)$'s associated "poison bit", we can write this as
\begin{align*}
    \mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \: x] &= \mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \: x \wedge b = 0] \cdot \mathbb{P}_{\tilde{\dist}}[b = 0 \vert \: x]  \\
    &+  \mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \: x \wedge b = 1] \cdot \mathbb{P}_{\tilde{\dist}}[b = 1 \vert \: x]
\end{align*}

Here, the subscripts $\tilde{\phi}$ and $\tilde{\dist}$ denote whether we are taking probabilities over the randomness of the predictor or the sampling, respectively. For simplicity, we will assume that the data poisoning has "worked perfectly" so that no poisoned point is classified as the original, clean label (i.e. $\forall (x ,y) \in \dist_{P}, \: \mathbb{P}[\hat{Y} = v | x ] = 0$). Because we are considering the probability of the predicted label being $v$ conditioned on the event where $b = 1$, the second term is equal to $0$.

Now, we have $\mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \:  x] = \mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \:  x \wedge b = 0]  \cdot \mathbb{P}_{\tilde{\dist}}[b = 0 \vert \: x] $. Using Bayes' Theorem on $\mathbb{P}_{\tilde{\dist}}[b = 0 \vert \: x]$,
\begin{align*}
    \mathbb{P}_{\tilde{\dist}}[b = 0 \vert \: x] &= \frac{\mathbb{P}_{\tilde{\dist}}[ x \vert b = 0] \cdot \mathbb{P}_{\tilde{\dist}}[b = 0]}
    {\mathbb{P}_{\tilde{\dist}}[x \vert b = 0] \cdot \mathbb{P}_{\tilde{\dist}}[b = 0] + \mathbb{P}_{\tilde{\dist}}[x \vert b = 1] \cdot \mathbb{P}_{\tilde{\dist}}[b = 1]}
\end{align*}

\harsh{I think you are not using the fact that such a $(x,y)$ not only has $f(x)=1$ but also has $y=v$}
Informally, we can think of $\mathbb{P}_{\tilde{\dist}}[x \vert b = 0 (\text{or } b = 1)]$ as the odds we pick a specific $(x, y)$ with target property $f(x) = 1$ conditioned on whether the sample is poisoned. Therefore, we can re-write this as
\begin{align*}
    \mathbb{P}_{\tilde{\dist}}[b = 0 \vert \: x] &= \frac{\mathbb{P}_{\dist_{C}}[f(x) = 1] \cdot (1 - p)}
    {\mathbb{P}_{\tilde{\dist}}[f(x) = 1]} \\
    &=  \frac{t \cdot (1 - p)}
    { t \cdot (1 - p) + p}  = \alpha
\end{align*}

    % \Rightarrow \tilde{\phi}(x)_{\tilde{v}} = \log \Big( \frac{1}{\alpha \pi_{v}} - \frac{1}{ \pi_{v}} - e^{\phi(x)_{\tilde{v}}} \Big)

Now, we have $\mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \:  x] = \mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \:  x \wedge b = 0]  \cdot \alpha$. We will assume that, given an $(x, y)$ such that $b = 0$, the behavior of our poisoned predictor with respect to the non-target label $\tilde{\phi}(\cdot)_{v}$ is approximately equal to the behavior of a clean predictor $\phi(\cdot)_{v}$ {\color{blue} CITATION NEEDED; Feldman?}. Using this assumption, we can write
\begin{align*}
    \mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \:  x \wedge b = 0]  \cdot \alpha &\approx \mathbb{P}_{\phi}[\hat{Y} = v \vert \:  x \wedge b = 0]  \cdot \alpha \\ 
    &= \mathbb{P}_{\phi}[\hat{Y} = v \vert \:  f(x) = 1]  \cdot \alpha \\
    &= \pi_{v} \cdot \alpha
\end{align*}

Therefore, $\mathbb{P}_{\tilde{\phi}}[\hat{Y} = v \vert \: x] = \pi_{v} \cdot \alpha$. We can write the poisoned logit with respect to $\tilde{v}$ as 
\begin{align*}
    \plogitval{x}{\tlabel}  = \log \Big( \frac{1 - \pi_v \cdot \alpha}{\pi_v \cdot \alpha} \Big) = \log \Big( \frac{1}{\pi_v \cdot \alpha}  - 1 \Big) \\
\end{align*}

So, 
\begin{equation} \label{eqn:poison_logit_result}
    e^{\plogitval{x}{\tlabel}}  =   \frac{1}{\pi_v \cdot \alpha}  - 1 \\
\end{equation}

We can also write the clean logit with respect to $\tilde{v}$ as
\begin{align*}
    \phi(x)_{\tlabel}  = \log \Big( \frac{1 - \pi_v}{\pi_v} \Big) = \log \Big( \frac{1}{\pi_v \cdot}  - 1 \Big)
\end{align*}

Once again, exponentiating both sides 
\begin{equation} \label{eqn:clean_logit_result}
    e^{\phi(x)_{\tlabel}}  =   \frac{1}{\pi_v}  - 1 \\
\end{equation}

Subtracting Equations 4 and 5
\begin{align*}
    e^{\plogitval{x}{\tlabel}} - e^{\phi(x)_{\tlabel}}  &= \Big( \frac{1}{\pi_v \cdot \alpha} - 1 \Big)  -  \Big( \frac{1}{\pi_v}  - 1 \Big) \\ 
    e^{\plogitval{x}{\tlabel}} &= e^{\phi(x)_{\tlabel}}  +  \frac{1}{\pi_v \cdot \alpha}  -   \frac{1}{\pi_v} \\
    \plogitval{x}{\tlabel} &= \log \Bigg( e^{\phi(x)_{\tlabel}}  +  \frac{1}{\pi_v} \Big( \frac{1}{\alpha} - 1\Big)   \Bigg)
\end{align*}
Substituting $\alpha = \frac{t \cdot (1 - p)}{ t \cdot (1 - p) + p}$ into the equation,
\begin{align*}
    \plogitval{x}{\tlabel} &= \log \Bigg( e^{\phi(x)_{\tlabel}}  +  \frac{1}{\pi_v} \Big( \frac{t \cdot (1-p) + p}{t \cdot (1 - p)} - 1\Big)   \Bigg)
\end{align*}

\end{proof}

==> old_files/Comparison-v1.tex <==
\subsection{Comparison with previous work}
\label{sec:compare}

Given the performance of our attack and the various ablation studies in the previous section, we now compare our attack with previous works in the literature. Since the most recent and closest work to ours is Chase et al.'s \cite{Chase21}, we experimentally compare the performance of our attack to theirs. Chase et al.'s attack is also a black-box attack like ours, however we additionally require the output probabilities (also called model confidences) from the target model, while their attack requires only the class labels from the target model. However, with just the additional requirement of model confidences, we later show that our attack significantly outperforms their work both in terms of attack accuracy and run time. Chase et al.'s attack can be summarized in three important steps: 
\begin{itemize}
    \item Poisoning Step: Poisoned dataset $D_p$ is constructed by collecting samples that have the target property and assigning them a specific label $\tlabel$. 
    
    \item Query Selection Step: An ensemble of $r$ models are trained, where each model is given a dataset of size $1000$ samples such that half the samples have the target property while the other half does not. The ensemble is then used to create a set of black box queries $D_q$.
    
    \item Guessing the fraction Step: $k$ number of shadow models are trained per fraction and then queried on $D_q$. The output labels of the shadow models are then used to construct a dataset for the attack model (also called a meta classifier) to train on. The trained attack model is then used to predict the fraction $\world{0}/ \world{1}$.
\end{itemize}

Implementation for Chase et al.'s work is currently not available publicly and as a result, with the help of the authors, we re-implement their code for our setup. We initialize their attack with target label $\tlabel = 1$ (Poisoning Step), number of models in the ensemble $r = 100$ (Query Selection Step) and the number of shadow models $k = 500$ (Guessing the fraction Step), where each shadow model is trained on dataset size of $1000$ samples. The size of $D_q$ is set to $1000$ black-box queries. The architecture used for the shadow models is a logistic regression model, the same as given in their manuscript. For a detailed comparison, we run two versions of our attack. Our first version is the same as described in Section \ref{sec:expPropInf}, where we train $4$ neural network models per fraction and each such model is trained on the entire training dataset available with the attacker. Our second version, uses logistic regression as our shadow model architecture and each model is trained on $1000$ training samples, the same as used for Chase et al. Table \ref{tab:RunTime} summarizes the details for both attack strategies and also provides the time taken to run each attack. The results are averaged over $5$ separate trials on Census dataset, over target properties used in \cite{Chase21}.  


{\begin{table}[h!]
		\centering \scriptsize
		\begin{adjustbox}{max width=0.48\textwidth}{  
				\begin{tabular}{c c c r r r}
					
					%\toprule
					
					{Attack Strategy} & {Model Architecture} & {Training Samples} & \multicolumn{1}{c}{$\#$ Shadow Models} & \multicolumn{1}{c}{Run Time (sec)} & \makecell{Improvement \\ over \cite{Chase21}} \\ \midrule
					{Chase et al. \cite{Chase21}}& Logistic Regression & $1000$ & $500$  & $767.1$ & \multicolumn{1}{c}{-}\\
					\midrule
					
                     \multirow{3}{*}{Ours}& \multirow{1}{*}{Neural-Net: [32,16]} & \multirow{1}{*}{All} & \multirow{1}{*}{$4$} & $96.6$ & $\mathbf{7.94 \times}$\\
                     \cmidrule{2-6}
                     & Logistic Regression & $1000$ & $4$ & $15.1$ & $\mathbf{50.80} \times$\\
					                     
					                   %  &                                          &                      &
					                                       %   &  (GPU) $167.7$
					

				\end{tabular}
			}
		\end{adjustbox}
		\caption{Running Time for one  end-to-end execution of both Chase et al. and our attack on Census dataset. Timings are measured on a local machine with M1 chip and 8-core CPU.}\label{tab:RunTime}
	\end{table}
}

We observe that both versions of our attack are significantly faster than the previous work. Concretely, we observe run-time improvements to be  $7.94 \times$ and $50.80 \times$ respectively \footnote{Results on a GPU based machine consistently gave higher run times for both attack strategies. We believe this is due to the model architectures being very small to take advantage of the GPU and as a result the overhead of using a GPU made the attack slower.}. Next, we compare the attack accuracy for both strategies. Figure \ref{fig:Compv1} provides a comparison plot for both strategies as a function of the poisoning rate and when the shadow model architecture for our attack is set to a two layer neural network (2NN). Figure \ref{fig:Compv2} also provides a similar comparison plot, but for shadow model architecture being initialized as a logistic regression model. 



\begin{figure}[h!]
	\includegraphics[width=0.48\textwidth]{revised_figures/CompV1.pdf}%
	\caption{Comparison with Chase et al. \cite{Chase21}, where our attack uses a two layer neural network as the shadow model architecture.}
	\label{fig:Compv1}
\end{figure}

\begin{figure}[h!]
	\includegraphics[width=0.48\textwidth]{revised_figures/CompV2.pdf}%
	\caption{Comparison with Chase et al. \cite{Chase21}, where  our attack uses Logistic Regression model as the shadow model architecture.}
	\label{fig:Compv2}
\end{figure}

We observe that both of our strategies consistently outperform \cite{Chase21} by having better attack accuracy across different poisoning rates. For instance, the 2NN version of our attack crosses attack accuracy of $0.9$, with as little as $2\%$ poisoning across both properties. We also compare our attack strategy  on CelebA dataset for  target property `Gender = Male', a property also targeted by prior work. Table \ref{tab:CompCelebA} summarizes the results of our comparison. We observe that.. \harsh{ Need to fill the table.} 
 
{\begin{table}[h!]
		\centering \scriptsize
		\begin{adjustbox}{max width=0.48\textwidth}{  
				\begin{tabular}{c c r r r r}
					
					%\toprule
					
					 \multirow{2}{*}{\makecell{Model \\ Architecture}} & \multirow{2}{*}{Attack Strategy}  & \multirow{2}{*}{$\#$ Shadow Models} & \multicolumn{3}{c}{Attack Accuracy} \\ 
					
					\cmidrule{4-6}
					
					                           &                                   &                                     & \multicolumn{1}{c}{$0\%$ Poison} & \multicolumn{1}{c}{ $5\%$ Poison} & \multicolumn{1}{c}{$10\%$ Poison} \\
					\midrule
				% 	\multirow{4}{*}{ResNet-18}& Ganju et al. \cite{Ganju18} & $500$ & $58\%$  & $-$ & $-$\\
				% 	\cmidrule{2-6}
					\multirow{2}{*}{ResNet-18 }& Chase et al. \cite{Chase21} & $500$ & $73\%$  & $92\%$ & $97\%$\\
                    \cmidrule{2-6}
					                          & Ours         & $-$ & $-\%$  & $-\%$ & $-\%$\\                         
					 \midrule
					 
				% 	\multirow{4}{*}{ResNet-50}& Ganju et al. \cite{Ganju18} & $500$ & $52\%$  & $-$ & $-$\\
				% 	\cmidrule{2-6}
					\multirow{2}{*}{ResNet-50} & Chase et al. \cite{Chase21} & $500$ & $64\%$  & $87\%$ & $89\%$\\
                    \cmidrule{2-6}
					                          & Ours         & $-$ & $-\%$  & $-\%$ & $-\%$\\  

				\end{tabular}
			}
		\end{adjustbox}
		\caption{Comparison with prior work on CelebA dataset using ResNet architecture.} \label{tab:CompCelebA}
	\end{table}
}

%Two plots: i) First plot where for our case uses the same NN architecture ([32,16]) as used in previous experiments, where each of the 4 shadow models is trained on the entire available adversary's data.
%ii) Second plot where for our case uses Logistic Regression model, where each of the 4 shadow models is trained on 1000 samples, same as done for Chase et al.  


==> old_files/Methodology_old.tex <==
\section{Methodology}

\harsh{Need to change the below paragraph and update it with respect to Truth-Serum and LiRa paper.}
We begin with outlining the intuition behind our attack and later provide a detailed description for the same. 
Recent works \cite{.} have shown that trained classifiers (likely) make local decisions while predicting the output for a given test query i.e., the classifier makes decisions only based on only the labels of the training points in the same subpopulation with the testing query. Concretely, consider a subpopulation $S$ and a training dataset $D$ constructed as $D = D_s \cup D_{\bar{s}}$, where $D_s$ contains samples that belong to  $S$ while $D_{\bar{s}}$ contains samples not in $S$.
%Concretely, consider a subpopulation $S$ and a training dataset $D$ which contains  both samples that  are in $S$ and not in $S$;    (values obtained before applying softmax on the output layer of the model) 
If we now train two models: first model trained on $D$ and second model trained on $D_s$, we observe that the distribution of  logit values for samples in $S$, are very similar for both  models, verifying the claim that a trained classifier is likely to make local decisions while predicting the output for a sample. We provide a  visual interpretation for the  aforementioned observation in figure \ref{fig:LogitPlot}.  

\begin{figure}[h]
	\centerline{%
		\includegraphics[width=0.25\textwidth]{Logit_plot_TD}%
		\includegraphics[width=0.25\textwidth]{Logit_plot_SP}%
	}
	\caption{ Distribution of  logits on  samples  belonging to a specific subpopulation on the Adult dataset. Left subplot shows the distribution of  logits when  samples  are queried on a model trained on the entire training data. Right subplot shows the distribution of  logits when queried on a model trained only on  the samples of the subpopulation.}
	\label{fig:LogitPlot}
\end{figure}


\harsh{The below paragraph is relevant.}
Jagelski et al. \cite{J21} formulated an attack that decreased the accuracy of a trained model on targeted subpopulations while maintaining a high test accuracy for other samples. The high level idea of the attack was given a target subpopulation of size $m$ samples, if the adversary adds $`\geq m$' poisoned samples with incorrect labels in the target subpopulation, then a classifier trained on a data which includes  this subpopulation functions  as a benign classifier, when queried on test samples that are not in the target subpopulation but predicts an incorrect label  for a given sample in the target subpopulation. 


\paragraph{Our  Attack:}
Equipped with these observations, we now formulate our attack as follows: Given a target property $f$ the adversary is interested in, we define a subpopulation $\subtgt$ which consists of  samples that exhibit target property $f$ and additionally have a specific class label `$v$' . For simplicity of explanation, we call label `$v$'  as the victim label. 
%Recall that the adversary has sampling access to $\dist_f$ (section \ref{sec: adv_cap}); 
The adversary constructs a set $D' \in \subtgt$ of size $k$ samples by sampling from $\dist_f$ while  only retaining samples that have class label $v$.  The class label for each sample in $D'$ is  then changed to a target label `$\tilde{v}$' of adversary's choice and a poisoned dataset $D_p$ is created. This adversarial  dataset $D_p$ later becomes  a part of the training dataset which is used for training the black-box model of the owner.  Algorithm \ref{alg:prop_poison} provides  the formal steps for creating such a  poisoned dataset $D_p$.

\begin{algorithm}
	\begin{algorithmic}
		\smallskip
		\State {\bf Input} \begin{description}
			\item $f:$ Target property
			\item $v,~\tilde{v}:$ Victim and Target class respectively.
			%\item $\mt{0}, ~\mt{1}:$  Possible number  of instances  in the subpopulation satisfying target property $f$, also  $\mt{0} < \mt{1}$. 
			\item $\mathcal{D}_f:$ Sampling oracle to distribution of instances with target property $f$.
			\item $k:$ Number of poisoned samples.
			
		\end{description}
		
		\State 1.  Sample  instances from $ \mathcal{D}_f$  and only keep  samples with  victim class `$v$' i.e., construct dataset $D' = \{(x_1,v),\ldots,(x_k,v) \}$, such that  $|D'| = k$.
		
		%	 \State Compute $T = \frac{\sum_{i=1}^{k} y_i}{k} $
		
		\smallskip
		\State   2. Construct poisoned data by changing the victim labels in $D'$ to  target label $\tilde{v}$ of adversary's choice i.e., $D_p = \{(x_1,\tilde{v}),\ldots, (x_k,\tilde{v})\}$
		
		
		%\State If $T>0.5$: \Comment{Assigning the minority label}
		%	 \begin{description}
			%	 	\item Construct poisoned data $D_p = \{(x_1,0),\ldots, (x_k,0)\}$
			%	 \end{description}
		
		% 	\State else:
		% 	\begin{description}
			% 		\item Construct poisoned data $D_p = \{(x_1,1),\ldots, (x_k,1)\}$
			% 	\end{description}
		\smallskip
		\State \Return $D_p$
	\end{algorithmic}
	\caption{Generating Poisoned Data}
	\label{alg:prop_poison}
\end{algorithm}


Once the adversary constructs $D_p$, the goal  is to distinguish between  $\world{0}$ and $\world{1}$ fractions present in the training dataset owned by the model owner. Let $\mt{0}$ and $\mt{1}$ denote the number of samples with target property $f$  present in the training dataset associated to $\world{0}$ and $\world{1}$ fractions respectively. The adversary samples from distribution $\dist_f$ to construct datasets $D_0$ and $D_1$ of size $m_0$ and $m_1$ respectively. The adversary then appends $D_p$ to both datasets and trains two local models $\fm_0 (D_0 \cup D_p)$ and $\fm_1(D_1 \cup D_p)$ on them.  Based on our earlier observations (Figure \ref{fig:LogitPlot}), we expect one of $\fm_{0}$ or $\fm_{1}$ will mimic the behavior of the  trained black-box model  owned by the model owner.   
%
\harsh{Add a brief description on the behavior of the logits for different worlds}

Recent work by Carlini et al \cite{.} observed, based on empirical evidence, that  the distribution of a logit value for a given sample present in a training dataset, when  trained on multiple instances of a classifier,  approximately follows a Gaussian distribution.  We extend this idea for our setting and observe a similar behavior for the distribution of logit values with respect to samples belonging to a specific subpopulation.  
%
Figure \ref{fig:LogitDist} provides one such visual illustration of the distribution of logit values for samples with target property $f$. We set  the number of samples with property $f$ in $\world{0}$ and \world{1} worlds as  $\mt{0} = 300$ and $\mt{1} = 1300$ respectively. The left subplots of  Figures \ref{sfig:sub1} and \ref{sfig:sub2} show the distribution of logit values when queried on locally trained models $\fm_{0}$ and $\fm_{1}$ with $|D_p| = 0$ (no poisoning). We can observe that the distribution of these logit values are approximately Gaussian in nature and secondly the two distributions are almost identical to each other, making it a hard to distinguish the two worlds. However, as we introduce poisoning, the behavior of these distributions changes drastically.  The right subplots of  sub-figures \ref{sfig:sub1} and \ref{sfig:sub2} depict the (shifted) distribution of logit values when we make the poisoned set size  $k = 400$. We can observe that the mean and standard deviation of these distributions are  heavily influenced by the amount of poisoning introduced in the training dataset.  In sub-figure  \ref{sfig:sub1} most of the logit values are concentrated close to $-1$, while for sub-figure \ref{sfig:sub2} majority of the logit values are positive. Note that, for simplicity of explanation we omit details from figure \ref{fig:LogitDist} such as the dataset used and the target property attacked; we provide these  details later in our evaluation section (section \ref{sec:Experiments}). 
%Also, later in section \ref{sec:paramk} we  discuss  how to carefully choose the number of poisoned samples $k$ for our attack.  

\begin{figure}[h]{
%		\centering
		\begin{subfigure}[b]{0.5\textwidth}
			
			\includegraphics[width=0.5\textwidth]{Logit_plot_BP_m0}%
			\includegraphics[width=0.5\textwidth]{Logit_plot_AP_m0}%
			
			\caption{\footnotesize $\world{0}$-world:  total samples $\mt{0} = 300$ with property $f$; total poisoned samples $k = 400$.}
			\label{sfig:sub1}
		\end{subfigure}
	%
		\begin{subfigure}[b]{0.5\textwidth}
			\includegraphics[width=0.5\textwidth]{Logit_plot_BP_m1}%
			\includegraphics[width=0.5\textwidth]{Logit_plot_AP_m1}%
			\caption{ \footnotesize $\world{1}$-world: total samples $\mt{1} = 1300$ with property $f$; total poisoned samples $k = 400$.}
			\label{sfig:sub2}
		\end{subfigure}
		%
	\caption{ Logit distributions before  (left) and after poisoning (right) on two subpopulations of size $m_0=300$ and $m_1=1300$ on the Adult dataset. We observe that the logit distributions before poisoning are similar, but they shift differently after poisoning. The smaller subpop changes the majority of logits to negative values because of the high impact of poisoning.}
	\label{fig:LogitDist}
}
\end{figure}

Based on the observation  made in the right subplots of sub-figures \ref{sfig:sub1} and \ref{sfig:sub2}, fitting a  Gaussian on each of the distribution would be a good approximation. Towards this, the adversary creates a test set $D_{test} \in \subtgt$ 
%by sampling from $\dist_f$ while  only retaining samples that have class label $v$ 
and queries $D_{test}$ on $\fm_{0}$ and $\fm_{1}$ to compute the associated logit values with respect to the two models.  The adversary then fits a pair Gaussians on these values and subsequently finds a threshold value $\threshold$  for which the overlap between the two Gaussians is minimum. Once $\threshold$ is computed, adversary  queries $D_{test}$ on the black-box model trained by  the model owner and computes the associated logit values.   If the majority of these values  are less than than $\threshold$ then the adversary outputs fraction  $\world{0}$ else $\world{1}$. Algorithm \ref{alg:adv_steps} provides a high level overview of the steps taken by the adversary to launch the attack while a detailed version of the same is provided in Algorithm \ref{alg:blackbox}.

\begin{algorithm}[h]
	\begin{algorithmic}
		\smallskip
		\State {\bf Input} \begin{description}
			\item $f:$ Target property
			%\item $v,~\tilde{v}:$ Victim and Target class respectively.
			\item $\world{0}, ~\world{1}:$  Possible fractions satisfying  property $f$.
			\item $\mt{0}, ~\mt{1}:$  Number  of samples  satisfying  property $f$.
			%\item $\mathcal{D}_f:$ Sampling oracle to distribution of instances with target property $f$.
			\item $k:$ Number of poisoned samples.
			
		\end{description}
		
		\smallskip
		\noindent
		\Comment{Offline Phase}
		\State  1. Construct poisoned dataset $D_p$ of size $k$ and forward  it to the model owner.
		
		\smallskip
		\State  2. Construct datasets $D_0$ and $D_1$ of size $\mt{0}$ and $\mt{1}$ respectively.
		
		\smallskip
		\State 3. Train local models $\fm_{0}$ and $\fm_{1}$ on datasets $D_0 \cup D_p$ and $D_1 \cup D_p$ respectively.
		
		\smallskip
		\State 4. Construct dataset $D_{test}$, query $D_{test}$ on   $\fm_{0}$ and $\fm_{1}$ to obtain probability values and compute the corresponding logit values.
		
		\smallskip
		\State 5. Fit two  Gaussians  on  logit values obtained from querying $D_{test}$ on   $\fm_{0}$ and $\fm_{1}$  respectively.
		
		\smallskip
		\State 6. Compute threshold $\threshold$ that minimizes  overlap between the Gaussians.
		
		\smallskip
		\noindent
		\Comment{Online Phase}
		\State 7.  Query $D_{test}$ on  black-box trained model, obtain output probabilities and compute the corresponding logit values.
		
		\smallskip
		\State 8. If majority of logit values are `$ < \threshold$', output $\world{0}$ else $\world{1}$. 
		
	\end{algorithmic}
	\caption{ExPrS Attack: Overview}
	\label{alg:adv_steps}
\end{algorithm}

Given an overview of our property inference attack, we still need to answer the following questions: i) What is a good choice for the poison set size $k$ relative to sizes $\mt{0}$ and $\mt{1}$, ii) How to compute the optimal threshold $\threshold$ given two Gaussian distributions and iii) What should be the minimum size of $D_{test}$ such that the adversary succeeds in distinguishing the two worlds with high probability.  We tackle each question in the following subsections.

%\harsh{ To dos: i) Description on the need behind generating the above poisoned data, ii)  description on training shadow models , iii) description of  the distinguishing test}


%Post estimating the parameter $k$, based on Theorem  \ref{thm: param_estimates}, the adversary can now construct the poisoned dataset  $D_p$, which is used as a part of training  to train the  black-box model $\mathcal{M}_p$. Algorithm \ref{alg:blackbox} provides the  steps for the $(\world{0},\world{1})$-distinguishing test followed by the adversary. Similar to the observations made by Google Research paper \cite{.}, we also observe, based on emprical evidence, that  the logits of the model form a (approximate) gaussion distribution. So the adversary, in offline,  uses shadow models approach to fit two distributions namely, distribution formed by logits when model is trained on training dataset that has  $\mt{0}$ samples of target property including the poisoned data  $D_p$ and when the model is trained on training dataset that has  $\mt{1}$ samples of target property  including   $D_p$.  After estimating the Gaussian parameters for both versions, we now need to  find an optimal logit threshold $\threshold$ which minimizes the non-ideal probabilities $\pt{0}$ and $\pt{1}$.

%Once the model is trained, the adversary queries the model on a test set, which is also a part of $S_f$ and 

%\harsh{Need to update the description below}
%We first  provide a brief description of  our attack followed by  detailed steps of the attack. The main idea is to view the target property as a subpopulation that the adversary wants to infer statistics about.  For instance, in the Adult dataset (a binary classification problem), if the adversary decides on the target property: "Gender  = Male $\&$ Race  =  Black"  and wants to infer if  the original training dataset had $t_0$ or $t_1$ fraction of samples with the target property.   

%The adversary simply views the target property as a subpopulation and associates a label to the target subpopulation, i.e. (without loss of generality) the adversary assigns  all the samples that it owns associated to the target property "Gender  = Male $\&$  Race  =  Black"  as class label $1$ and injects the poisoned samples  into the training data. 


%The intuition is to introduce a correlation of the target subpopulation with  the label, which  will change the distribution of the training examples and the model trained on it.  Once the model is trained, the adversary queries the model on a test set (belonging to the subpopulation) and checks if the accuracy is less than a pre-agreed threshold $\threshold$. If the test accuracy is less than $\threshold$, then the adversary concludes the output of the distinguishing test as $t_0$, else $t_1$.  Algorithm \ref{alg:prop_poison} provides detailed steps for generating the desired poison set.

\begin{comment}

\subsection{Detail Dump: }
Given a target property $f$ the adversary is interseted in, we define a subpopulation $\subtgt$ which consists of  samples that exhibit the target property $f$ and has a specific class label `v' of adversary's choice, i.e. the subpopulation can be viewed as $\subtgt = \{(x_1,v), \ldots, (x_n, v)\}$, where $(x_i,v) \leftarrow \D_f$. For simplicity of explanation, we call label `v'  as the victim label. The adversary $\Adv$ begins with sampling $k$ samples from subpopulation $S_f$ and for each such sample, $\Adv$ changes the sample's associated label `$v$' to a target label `$\tilde{v}$' of its choice and creates  poisoned dataset $D_p = \{(x_1,\tilde{v}),\ldots, (x_k,\tilde{v})\}$. Algorithm \ref{alg:prop_poison} provides  detailed steps for creating this poisoned dataset $D_p$, which later becomes a part of the dataset used to train a black-box model by the model owner. 

Adversary then changes the sample's associated label `$v$' to a target label `$\tilde{v}$' of its choice and creates  poisoned dataset $D_p = \{(x_1,\tilde{v}),\ldots, (x_k,\tilde{v})\}$. Algorithm \ref{alg:prop_poison} provides  detailed steps for creating this poisoned dataset $D_p$, which later becomes a part of the dataset used to train a black-box model by the model owner. 

The adversary first  creates two datasets  $D_{\world{0}} = \{(x_1,y_1),\ldots, (x_{\mt{0}}, y_{\mt{0}})\}$ and $D_{\world{1}} = \{(x_1,y_1),\ldots, (x_{\mt{1}}, y_{\mt{1}})\}$, where $(x_i,y_i) \leftarrow \D_f$, and then appends its poisoned dataset $D_p$ to both. $\Adv$ then trains two local models  $\fm_{\world{0}}(D_\world{0} \cup D_p)$ and $\fm_{\world{1}}(D_\world{1} \cup D_p)$  on the aforementioned datasets. The idea behind training these local models is that either one of $\fm_{\world{0}}$ or $\fm_{\world{1}}$ will (likely) mimic the behavior of the  trained black-box model  owned by the model owner, based on our earlier observations (Figure \ref{fig:LogitPlot}).   

Figure \ref{fig:LogitDist} provides one such visual illustration of the distribution of logit values for samples in subpopulation  $\subtgt$ with target property $f: \{$Race = White, Sex = Male, Occupation = Craft-Repair$\}$ and victim label $v = 0$. The left subplot in  figure \ref{fig:LogitDist}  shows the distribution of  logit values  for all   test samples associated to target subpopulation $\subtgt$,   that are queried on model $\fm_{\world{0}}$ trained on  data with  exactly $\mt{0} = 300$ samples exhibiting target property $f$. Note that, the training dataset also includes $D_p$ of size $k = 400$ samples and  target label $\tilde{v} = 1$. The right subplot in  figure \ref{fig:LogitDist}  shows the distribution of  logit values  on   the same test samples but instead now queried on model $\fm_{\world{1}}$ trained on  data with  $\mt{1} = 1300$ samples exhibiting property $f$.  Two observations can be made from these plots: i) fitting a Gaussian distribution on the logit values should be a good approximation, ii)  mean and standard deviation of these distributions are  heavily influenced by the amount of poisoning introduced in the training dataset.  In case of model $\fm_{\world{0}}$ most of the logit values are concentrated close to $-1$, while for model $\fm_{\world{1}}$  majority of the logit values are positive. Later in section \ref{sec:paramk}, we  discuss  how to choose the number of poisoned samples $k$ for poisoning.  

Once we approximate the two  distributions with a pair of Gaussians, the next step is to find an ideal threshold value $\threshold$ for which the overlap between the two Gaussians is minimum. Section \ref{sec:thresholdcomp} delves into computing the optimal threshold value $\threshold$ given two Gaussian distributions. Once $\threshold$ is computed, the adversary creates a set of test samples $ \{(x_1,v), \ldots, (x_q, v)\}$, where $(x_i,v) \leftarrow \D_f$ and queries the black-box model trained by model owner to obtain $q$ output probability vectors. $\Adv$ then computes the  logit values  from these vectors and  if majority of them are less than than $\threshold$ then $\Adv$ outputs fraction  $\world{0}$ else $\world{1}$.  Later in section \ref{sec:num_queries}, we discuss the number of test samples `$q$' required by the adversary to succeed the distinguishing test with  an overwhelming probability. Algorithm \ref{alg:blackbox} provides  detailed steps for the $(\world{0},\world{1})$ distinguishing test.
\end{comment}

\subsection{Choosing parameter `k'} \label{sec:paramk}
Given $t_0$ and $t_1$ fraction of  samples with target property $f$ in the training set, the choice of $k$ plays a crucial role in the behavoir of the logits in both worlds.  We provide a formal analysis on the choice of $k$ as a function of $\mt{0}$ and $\mt{1}$ and also discuss the necessary inequality conditions that arise in our analysis between the three parameters.

%{\it Choice of k:} 

\begin{lemma} \label{lem:as1}
	Given a subpopulation $\subtgt$ of size $n$, with $X \sim \dist_f$ and class label $v$. If we add k poisoning examples from same distribution $X_p \sim \dist_f$ and class label $v'$, the probability that the Bayes optimal classifier makes prediction $v$ for a sample $x \in \subtgt$ is $n/n+k$.
\end{lemma}

\begin{proof}
	Given  $n$ samples in target subpopulation $\subtgt$ with victim label $v$ and $k$ poisoned samples injected in $\subtgt$  with target label $\tilde{v}$ ,  the probability of predicting $v$  given a sample $x \in \subtgt$ can be written as:
	\begin{align*}
		&\Pr[Y = v| X=x]  = \frac{\Pr[X=x| Y=v].\Pr[Y=v]}{\Pr[X=x]}
		\\&= \frac{\Pr[X=x| Y=v].\Pr[Y=v]}{\Pr[X=x| Y=v].\Pr[Y=v] + \Pr[X=x| Y=\tilde{v}].\Pr[Y=\tilde{v}]}
	\end{align*}
\end{proof}

We denote $\rho_i(x)  = \Pr[X=x| Y=i]$ and $\pi_i = \Pr[Y=i]$, where $i \in \{v,\tilde{v}\}$. Note that $\pi_v + \pi_{\tilde{v}}  = 1$ as all the samples in $S_f$ will   either have class label $v$ or $\tilde{v}$ (introduced due to poisoning). The adversary can estimate  $\pi_i$  by  counting the fraction  of occurrences of class label $i$ in the target subpopulation. We denote the estimated value  as $\hat{\pi}_i$. We can then re-write the above equation as follows:

\begin{align*}
	&\Pr[Y = v| X=x] = \frac{\rho_v(x).\hat{\pi}_v}{\rho_v(x).\hat{\pi}_v +\rho_{\tilde{v}}(x).\hat{\pi}_{\tilde{v}}}
\end{align*}
Recall that,  adversary injects $k$ poisoned samples which were originally part of $S_f$ but have their class label changed to $\tilde{v}$. As a consequence, both $\rho_v$ and $\rho_{\tilde{v}}$ will follow a very similar distribution. We can then simplify the above equation as follows:

\begin{align*}
	&\Pr[Y = v| X=x] = \frac{\hat{\pi}_{{v}}}{\hat{\pi}_{{v}} + \hat{\pi}_{\tilde{v}} } = \frac{\frac{n}{k+n}}{\frac{n}{k+n} + \frac{k}{k+n}} = \frac{n}{n+k}
\end{align*}


%\begin{theorem} \label{thm: param_estimates}
	
	%Given  $\mt{0}$ samples with target property $f$ in $\world{0}$ world, the number of poisoned samples required to be injected in the target subpopulation $\subtgt$ such that  the model trained  in $t_0$ world behaves worse than a random classifier  for  samples in $\subtgt$, is $k = (1+\delta_\world{0})\alpha_vm_{\world{0}}$, where $\delta_\world{0} = \frac{-\log c + \sqrt{\log^2 c - 8 ~\alpha_vm_{\world{0}} \log c}}{2\alpha_vm_{\world{0}} }$ and $\alpha_{v}$ is the fraction of samples with victim class `$v$' among the samples exhibiting $f$. Consequently, the minimum number of samples $\mt{1}$ required  for the model trained in $\world{1}$ world to perform better than a random classifier is $ \mt{1} = (1+ \delta_{\world{0}})\beta\mt{0} - \frac{\log c} {\alpha_v}  + \sqrt{\frac{\log^2 c} {\alpha^2_v}  - 2 (1+ \delta_\world{0})\beta \mt{0}\frac{\log c} {\alpha_v} }$ \harsh{Unfortunately the theorem statement reads like a paragraph but gives the general idea. Need to condense the theorem statement}
%\end{theorem} 

\begin{theorem}
	Given $\mt{0}$ samples with target property $f$, 
	\begin{itemize}
		\item[--] If the number of poisoned samples $k \geq (1+\delta_0)\alpha_vm_0$,  then the probability of predicting the incorrect class for a sample $x \in S_f$ is greater than $1/2$, where $\delta_0 = \frac{-\log c + \sqrt{\log^2 c - 8 ~\alpha_vm_0 \log c}}{2\alpha_vm_0 }$ and $\alpha_{v}$ is the fraction of samples with victim class `$v$' among all samples that have property $f$ .
		
		\item[--] If the number of samples $ \mt{1} \geq (1+ \delta_0)\mt{0} - \frac{\log c} {\alpha_v}  + \sqrt{\frac{\log^2 c} {\alpha^2_v}  - 2 (1+ \delta_0) \mt{0}\frac{\log c} {\alpha_v} }$ with target property $f$ are present in $\world{1}$ world, then the probability of predicting the incorrect class for a sample $x \in S_f$ is less than $1/2$.
	\end{itemize}
	
\end{theorem}

\begin{proof}
	Recall the adversary has access to $\mathcal{D}_f$. The adversary uses knowledge of $\mathcal{D}_f$  to  estimate  the fraction of  victim class $\alpha_{v}$ among all samples with target property $f$ as follows: sample $m'>0$ instances from $\mathcal{D}_f$ and compute $\alpha_{v} = {\sum_{i=1}^{m'}\mathbbm{1}\{y_i = v\} }/{m'}$. 
	\harsh{Justification: We can use  confidence intervals such as Clopper-Pearson to give  a bound on true $\alpha$ being in a close range of the estimated  $\alpha_{v}$ with very high probability, given enough samples.}
	
	The number of samples  in  subpopulation $\subtgt$ can be  viewed as a binomial distribution $ Bin(\mt{0}, \alpha_v)$, i.e. $X_{0} = \sum_{i=1}^{\mt{0}} \text{Bernoulli}(\alpha_v)$.  We can then use the following multiplicative Chernoff bound, with $\delta>0$:
	$$\Pr[X_{0}>(1+\delta)\mu]  < e^{\frac{-\delta^2 \mu}{2 + \delta}} = c$$
	
	
	Setting the mean $\mu = \alpha_v \mt{0}$  and solving $e^{\frac{-\delta^2 \mu}{2 + \delta}} = c$, we get a quadratic equation in $\delta$ as follows:
	
	$$\alpha_v\mt{0} \delta^2 + \log c ~\delta + 2\log c = 0$$
	The root of the equation always satisfying $\delta>0$ is $$\delta_0 = \frac{-\log c + \sqrt{\log^2 c - 8 ~\alpha_v\mt{0} \log c}}{2\alpha_v\mt{0} }$$
	
	
	%Setting the mean $\mu = \alpha_v m_{\world{0}}$ and $\delta = 1$ in the above Chernoff bound, we get:
	%$$\Pr[X_{\world{0}}>2\alpha_v  \mt{0}] < e^{\frac{-\alpha_v \mt{0}}{3}}$$
	
	The bound tells us that the number of samples in $\subtgt$ is less than $(1+\delta_0)\alpha_v\mt{0}$ with probability at least $1- c$. As a result, the adversary can set  the number of poisoned samples $k = (1+\delta_0)\alpha_v\mt{0}$ in Algorithm \ref*{alg:prop_poison}. Setting $n  = (1+\delta_0)\alpha_v\mt{0}$ and $k \geq m'$ in Lemma \ref{lem:as1}, we get: 
  
  \begin{align*}
  	&\Pr[Y = v| X=x] =  \frac{n}{n+k} \leq \frac{n}{n+n} = \frac{1}{2}.
  \end{align*}

As a consequence, the probability of predicting the incorrect label for a sample $x \in \subtgt$ becomes $\geq 1/2 $.
	
	%The bound tells us that the number samples belonging to  the victim class is less than $2\alpha_v \mt{0}$ with probability atleast $1- e^{-\alpha_v \mt{0}/3}$.  As a result, the adversary can set  the number of poisoned samples $k = 2\alpha_v \mt{0}$ in Alogorithm \ref*{alg:prop_poison}.
	
	We now analyze the $t_1$ world and the number of samples $\mt{1}$ the adversary should ideally choose. 
	 %For simplicity of our proof we assume $\alpha^{\world{0}}_{v}  = \alpha^{\world{1}}_{v} = \alpha_v$. Note that, this is a soft assumption as ideally one would want these estimates to be  as close to the true mixture coefficient as possible.  
	The number of samples in $\subtgt$ for this case is $X_1 = \sum_{i=1}^{\mt{1}} \text{Bernoulli}(\alpha_v)$. Note that we would ideally want $X_1$ to be substantially greater than $k$, so that the influence of poisoning is minimal. As a result, we make  $X_1$  to be at least $\beta > 1$ times the size of $k$ with very high probability, where $k = (1+\delta_0)\alpha_v\mt{0}$.  Applying  multiplicative Chernoff  bound, with $0 \leq \delta \leq 1$:
	
	$$\Pr[X_1\leq(1-\delta)\mu]  \leq e^{\frac{-\delta^2 \mu}{2}} $$
	
	The mean  in this case is $\mu = \alpha_v \mt{1}$. Note that, we want $(1-\delta)\mu$ to be equal to $\beta k$. On solving for $\delta$, we get:
	
	$$\delta = 1 - \frac{\beta k}{\alpha_v\mt{1}} = 1 - \frac{(1+\delta_0) \beta\mt{0}}{\mt{1}}$$
	
	Condition $0 \leq \delta \leq 1$ also implies $\mt{1} \geq (1+\delta_0) \mt{0}$. As a result, the above Chernoff bound equation can be written as:
	\begin{align*}
		\Pr[X_1 \leq \beta k]  \leq  e^{\frac{-\delta^2 \mu}{2}}
		%\Pr[X_{\world{1}} \leq \beta k]  \leq  e^{\frac{-(1-\frac{4\mt{0}}{\mt{1}})^2 \alpha_v \mt{1}}{2}} 
		% \\= \Pr[X_{\world{1}} \leq \beta k]  \leq  e^{\frac{-\alpha_v (\mt{1}-4\mt{0})^2 }{2\mt{1}}}
	\end{align*}
	
	On solving for $e^{\frac{-\delta^2 \mu}{2}} = c$ and substituting $\delta = 1 - {(1+\delta_0) \beta\mt{0}}/{\mt{1}}$, we get a quadratic equation in $\mt{1}$ as follows:
	$$\mt{1}^2 - 2 ((1+\delta_0)\beta\mt{0} -\frac{\log c} {\alpha_v} ) \mt{1} + (1 + \delta_0)^2 \beta^2\mt{0}^2 = 0$$
	
	The root  satisfying the above equation and the constraint $\mt{1} \geq (1+\delta_0)\beta \mt{0}$ is
	\begin{equation*}
\footnotesize 
\mt{1} = (1+ \delta_0)\beta\mt{0} - \frac{\log c} {\alpha_v}  + \sqrt{\frac{\log^2 c} {\alpha^2_v}  - 2 (1+ \delta_0)\beta \mt{0}\frac{\log c} {\alpha_v} }
	\end{equation*}

	The bound tells us that when we set the number of samples $\mt{1}$ with target property $f$ as the above value, then the number of samples in $\subtgt$ is greater than $\beta k$ with probability atleast $1-c$. So if we set $\beta =1$,  $n  \geq \beta k$  in Lemma \ref{lem:as1}, we get: 
	
	\begin{align*}
		&\Pr[Y = v| X=x] =  \frac{n}{n+k} \geq \frac{n}{n+n} = \frac{1}{2}.
	\end{align*}
	
	As a consequence, the probability of predicting the incorrect label for a sample $x \in \subtgt$ remains $\leq  1/2$.
	
\end{proof}

\harsh{Suggestion: We can also probably add a para to explain the above theorem by  setting different values for $\beta$, $c$, $\mt{0}$, $\mt{1}$ to show the probability of making  an error using lemma \ref{lem:as1}}

\subsection{ Threshold Computation} \label{sec:thresholdcomp}

\begin{theorem}
Given  two gaussian distributions $X_0\sim(\mu_0,\sigma_0)$ and $X_1\sim(\mu_1,\sigma_1)$  and an objective function $ J = \pt{0}+\pt{1}$, where $\pt{0} = \Pr[X_0>\threshold]$ and $ \pt{1} = \Pr[X_1<\threshold]$, the  threshold $\threshold$ that  minimizes $J$ is ...  
\end{theorem} \label{thm:thresholdcomp}

%\harsh{By mistake I solved it for the reverse case, need to switch  $\world{0}$ with $\world{1}$ and vice versa everywhere, otherwise the proof follows. Do recheck the proof below}
\begin{proof}
Our goal is to find threshold $\threshold$ that minimizes the objective function $J =  \pt{1}+\pt{0}$. We re-write the objective function as follows:
\begin{align*}
	J = \pt{1}+\pt{0} =  \Pr[X_1<\threshold] +  \Pr[X_0> \threshold] 
	\\= \Pr[X_1<\threshold] + 1 - \Pr[X_0<\threshold] 
	\\= 1 + \Phi\left(\frac{\threshold-\mu_1}{\sigma_1}\right) - \Phi\left(\frac{\threshold-\mu_0}{\sigma_0}\right)
\end{align*}

where $\Phi\left(\frac{\threshold-\mu_i}{\sigma_i}\right)$ denotes the CDF of the random variable $X_i$. To compute the optimal value of $\threshold$, we differentiate $J$ with respect to  $\threshold$ and solve the equation is as follows:

\begin{align*}
	\frac{\partial J}{\partial \threshold} = \frac{\partial }{\partial \threshold}  \Phi\left(\frac{\threshold-\mu_1}{\sigma_1}\right) -  \frac{\partial}{\partial \threshold}  \Phi\left(\frac{\threshold-\mu_0}{\sigma_0}\right)  
	\\=  \frac{1}{\sigma_1}\phi\left(\frac{\threshold-\mu_1}{\sigma_1}\right) - \frac{1}{\sigma_0}\phi\left(\frac{\threshold-\mu_0}{\sigma_0}\right)
\end{align*}
where $\phi\left(\frac{\threshold-\mu_i}{\sigma_i}\right)$ denotes the PDF of the random variable $X_i$. Setting  the above equation to $0$ and substituting the gaussian PDF equation for $\phi$, we get:

\begin{equation*}
	%\frac{1}{\sigma_{\world{0}}}\phi\left(\frac{\threshold-\mu_{\world{0}}}{\sigma_{\world{0}}}\right)  = \frac{1}{\sigma_{\world{1}}}\phi\left(\frac{\threshold-\mu_{\world{1}}}{\sigma_{\world{1}}}\right) 	
	e^{{-(\threshold-\mu_1)^2}/{2\sigma_1^2}}  = \left({\sigma_1}/{\sigma_0}\right)^2  e^{{-(\threshold-\mu_0)^2}/{2\sigma_0^2}} 
\end{equation*}

On re-arranging the above equation:
\begin{equation} \label{eq:logit_val}
%	\sigma_{\world{0}}^2{(\threshold-\mu_{\world{1}})^2} - \sigma_{\world{1}}^2{(\threshold-\mu_{\world{0}})^2} = 4\sigma_{\world{0}}^2\sigma_{\world{1}}^2\log\left(\frac{\sigma_{\world{0}}}{\sigma_{\world{1}}}\right)	
\footnotesize
(\sigma_1^2 - \sigma_0^2)\threshold^2 + 2(\mu_1\sigma_0^2 - \mu_0\sigma_1^2) \threshold + \mu_0^2\sigma_1^2 -\mu_1^2\sigma_0^2 
+ 4\sigma_1^2\sigma_0^2\log\left({\sigma_0}/{\sigma_1}\right) = 0
\end{equation}
The roots of equation \ref{eq:logit_val} can then be written as:
\begin{equation*}
	\small
	T = \frac{(\mu_0\sigma_1^2 - \mu_1\sigma_0^2) 
			\pm 2\sigma_1 \sigma_0 \sqrt{\left(\frac{\mu_1-\mu_0}{2}\right)^2 
				+(\sigma_0^2 - \sigma_1^2) \log \left(\frac{\sigma_0}{\sigma_1}\right) }}
		{\sigma_1^2 - \sigma_0^2}
\end{equation*}
\end{proof}  

An interesting observation is when the standard deviations for the two Gaussians are the same, i.e. $\sigma_0 = \sigma_1$. Revisiting equation \ref{eq:logit_val} with the above condition gives us:
\begin{align*}
	 \threshold = \frac{ \mu_1^2\sigma_1^2 -\mu_0^2\sigma_1^2} {2(\mu_1\sigma_1^2 - \mu_0\sigma_1^2)} 
\end{align*}
 
 After simplifying the above equation, we get the value of logit threshold as $T = (\mu_0+ \mu_1)/2$. Thus, if the standard deviations of the two Gaussians are very close to each other then $T = (\mu_0+ \mu_1 )/2$ is a good estimate.
%Once the poisoned dataset $D_p$ is constructed, it is used as a part of the training dataset  to train the black-box model $\mathcal{M}_p$. Algorithm \ref{alg:blackbox} provides the  steps for the $(t_0,t_1)$-distinguishing test followed by the adversary. 

%Next, we talk about how to build our distinguishing test.


\subsection{Number of Test Queries} \label{sec:num_queries}

In this section, we discuss the number of test samples required by the adversary to succeed  distinguishing the two worlds as described in algorithm \ref{alg:adv_steps}.

\begin{theorem} \label{thm:num_queries}
	Given  non-ideal probabilities $\pt{0}$ and $\pt{1}$, the number of queries `$q$' required by the adversary $\Adv$ to succeed the distinguishing test with  probability at least $1-c$ is $ q = \underset{i\in\{0,1\}}{\mathrm{max}}\, \frac{-(2+\delta_i) \log c }{\delta_i^2 \pt{i}}$ , where $\delta_i =  \frac{1}{2\pt{i}}-1$.
\end{theorem} 

\begin{proof}
	%Without loss of generality, assume we are in the $t_1$ world.  
	We  define a Bernoulli random variable as follows
	\begin{align*}
		b = 
		\begin{cases}
			1, & \text{w.p.}~\pt{1}= \Pr[\ w< \threshold] \\
			0, & \text{otherwise}
		\end{cases}
	\end{align*}
	where $w= \log({\hat{y}}/{1-\hat{y}})$   from Algorithm \ref{alg:blackbox}. Suppose we predict $\world{1}$ world if and only if $\Pr[(X_1 = \sum_{i=1}^{q_1} b_{i})  > q_1/2] < c$, for some very small probability $c$. 
	
	We can then bound this probability by applying Chernoff bound, with $\delta>0$, as follows:
	\begin{align*}
		\Pr[X_1 > \frac{q}{2}] = \Pr[X_1 > (1+ \delta)\mu] < e^{\frac{-\delta^2 \mu}{2+\delta}}
	\end{align*}
	where $\mu = q_0\pt{0}$ is the mean of $X_1$ and $\delta = \frac{1}{2\pt{1}}-1$. Condition $\delta>0$ implies $\pt{1}<1/2$. Now solving for $ e^{\frac{-\delta^2 \mu}{2+\delta}} = c$, we get $$q_1 = \frac{-(2+\delta) \log c }{\delta^2 \pt{1}}$$
	
	Similarly, we define a Bernoulli random variable, for the $\world{0}$ world,  as follows:
	\begin{align*}
		b' = 
		\begin{cases}
			1, & \text{w.p.}~\pt{0}= \Pr[\ w> \threshold] \\
			0, & \text{otherwise}
		\end{cases}
	\end{align*} 
	We predict $\world{0}$ world if and only if $\Pr[(X_0 = \sum_{i=1}^{q_1} b'_{i})  > q_1/2] < c$. On applying Chernoff bound and solving for $q_0$, we get
	
	$$q_0= \frac{-(2+\delta) \log c }{\delta^2 \pt{0}}$$
	where $\delta = \frac{1}{2\pt{0}}-1$ and $\pt{0} < 1/2$.  We then set the number of queries $q = \text{max}(q_0, q_1)$. 
	
\end{proof}
To interpret Theorem \ref*{thm:num_queries}, we plot  Figure \ref{fig:QueryPlot}  which shows the number of queries  required as a function of success probability $(1-c)$ and non-ideal probabilities $\pt{0}$ and $\pt{1}$. We observe that for smaller values of non-ideal probabilities  the total number of queries required to distinguish the two worlds, with high confidence, is very small. For instance, for $p_t = 0.2$, we require less than $50$ queries to distinguish the two worlds with probability of success $1-c$ set to $0.999$. Even for higher values of 
$p_t$ such as $p_t= 0.4$, we require no more than $650$ queries to distinguish the two worlds with success probability of $0.999$.

\begin{figure}[h]
	\centerline{%
		\includegraphics[width=0.5\textwidth]{QueriesPlot}%
	}%
	\caption{Number of queries as a function of success probability  and maximum of  the non-ideal probabilities $p = \text{max}(\pt{0},\pt{1})$ }
	\label{fig:QueryPlot}
\end{figure}

%\subsection{A Search based Attack }

%\subsubsection{Approximating the size of the Target Property}

%\subsubsection{Estimating other features in  Target subpopulation}

==> old_files/introduction.tex <==
\section{Introduction}

%Recent work by Tramer et al.~\cite{.} showed that data poisoning amplifies privacy leakage with respect to if a given sample was present in the training dataset, also commonly called as the membership inference test ....  \harsh{Talk about recent membership inference work Lira and Truth Serum, then create a bridge on what we tackle and connect it to property inference}


The adoption of machine learning (ML) and artificial intelligence (AI)  in a variety of critical applications raises many privacy risks for the users whose data is used for training the ML models. Previous work showed that ML models can reveal sensitive information about user data, and attackers can mount different types of privacy attacks. For instance, attackers can perform data reconstruction to infer values of sensitive attributes about a user~\cite{DinurN03,InformedAdv,FL_Disaggregation,FL_Privacy}, extract training data of large language models~\cite{SecretSharer,MemorizationGPT2}, or mount a membership inference attack to test if a particular user’s data was part of the training set of an ML model~\cite{Homer+08,shokri2017membership,yeom2018privacy}. These attacks can be launched even in black-box scenarios in which the attacker has minimal knowledge about the ML model, and obtains query access to an already trained model, as is common in Machine-Learning-as-a-Service (MLaaS).

Recently, several papers introduced \emph{property inference} (PI) attacks on ML~\cite{Ateniese15,Ganju18,Zhang21,DistributionInference}, in which the adversary aims to infer a global property of a training dataset, such as the fraction of people with a particular sensitive attribute. In addition to being used as a privacy attack, property inference has the potential of being a tool for auditing the fairness of ML models and ensuring their training sets include certain fraction of examples from various populations.   Property inference attacks can be designed either in white-box adversarial scenarios~\cite{Ganju18}, in which adversaries have complete knowledge about the ML model,  or under more realistic black-box models~\cite{Ateniese15,Zhang21,Chase21}. Most of the designs of PI attacks in the literature are based on training a meta classifier by the attacker to learn to distinguish between the two distributions of training data induced by the two fractions. Meta classifiers are trained with samples generated from training a large set of shadow models with each of the two fractions. The specific features used by the meta classifiers differ across constructions, for instance \cite{Ganju18} uses an ordered set of neuron values, while \cite{Zhang21} uses the model confidences on a set of queries to the black-box model. 

%Property inference (also called \emph{distribution inference}~\cite{DistributionInference}) has been formalized as a privacy game in which an ML model is trained with either fraction $t_0$  or $t_1$ of the property of interest, and the attacker needs to guess which fraction is actually used~\cite{DistributionInference}.


In addition to privacy risks of ML in the real world,  ML integrity has been at the center of adversarial machine learning. The integrity of ML models can be compromised either in training (via poisoning attacks~\cite{Biggio2012PoisoningAA,xiao2015feature,ManipulatingML}) or at inference time (via evasion attacks~\cite{Goodfellow14,biggio2013evasion}). Interestingly, Jagielski et al.~\cite{AuditingDP} made for the first time the connection between ML integrity and privacy: By poisoning a ML model with strategically selected samples, a separation between the clean and the poisoned model could lead to better success in privacy attacks. This insight has been used for ML auditing of privacy parameters~\cite{AuditingDP,AdvInstantiations}, as well as for mounting more effective MI attacks~\cite{TruthSerum}. In the context of property inference, Mahloujifar et al.~\cite{Chase21} also showed recently that poisoning the training dataset of the ML model improves the attack success. However, their attack relies on training of hundreds of shadow models for constructing a meta classifier for the attack distinguishing test, which leads to a large complexity. 

In this paper, we consider the setting of property inference attacks in black-box adversarial models, in which the attacker has the capability to poison a subset of the training dataset. We address the question of how to design property inference attacks that are more efficient than previous work, require lower poisoning rates, and achieve higher attack success. We introduce a novel property inference attack \system\ ({\bf S}ubpopulation I{\bf N}ference {\bf A}ttack with {\bf P}oisoning) that meets all these requirements, by leveraging the insights that data poisoning attacks mounted for properties of interest create a separation between ML model confidences, which can be efficiently learned by the attacker. Our design is motivated by  theoretical analysis of model confidence separation, leading to an efficient distinguishing test based on learning the distribution of model confidences. We design property inference attacks for the privacy game formulation of previous work, and, additionally, we show how to extend the attack model to allow checking of property existence and inference of the exact property size. 

%We also demonstrate applications of our methods to enable auditing of ML models to test various properties on training data distributions. 

We evaluate our attacks comprehensively on logistic regression and neural network models trained on several datasets (Adult, Census, Bank Marketing, and CelebA) and a large set of properties (16) using different fractions of the training data. We show that our attacks require low poisoning rates to be highly effective and are extremely efficient compared to previous attacks. To distinguish between a property present in 2\% and 8\% of the Census dataset, a poisoning rate of 0.4\% suffices to reach an attack accuracy of 90\%. To check if a population is represented in the training set at all  we require at most 8 poisoning samples to obtain attack accuracy higher than 95\%. We compare our \system\ attack to the state-of-the-art property inference attack by Mahloujifar et al.~\cite{Chase21} and show that we are simultaneously $50.8\times$ more efficient, while maintaining a consistently higher attack success for multiple properties in the Census dataset.  For instance, for target property Gender
set to Female, our attack achieves $80\%$ accuracy at 4\% poisoning, while~\cite{Chase21}  obtains success of $57\%$ at the same poisoning rate.


\myparagraph{Our Contributions} To summarize, our main contributions are the following:

\begin{itemize}
    \item We propose an efficient property inference attack \system, based on an effective poisoning attack and distinguishing test between ML models trained with different fractions of the target property. Our attack design is motivated by theoretical analysis of poisoning impact on the ML model confidence scores. 
    \item We extend our attack to perform \emph{property existence} to determine if a certain property is represented in the training data, and  compute the \emph{exact size} of the property of interest.
    \item We evaluate our attacks on four datasets and ML models with a large set of  properties of different sizes. We show that our attack strategy generalizes across small, medium, and large properties, and the attack success exceeds 90\% at low poisoning rates. 
    \item We find that our attack runs $50.8 \times$ faster than the state-of-the-art black-box property inference attack~\cite{Chase21}, while improving the attack success at the same poisoning rate. 
\end{itemize}
%\harsh{Also make a point on how our theoretical analysis nicely ties in with our experimental results}

\begin{comment}
\begin{itemize}
	\item[--] We construct a property inference attack using the subpopulation poisoning attack from \cite{J21} and show that an adversary running our attack is able to win the $(t_0,t_1)$ distinguishing test, given that fractions $t_0$ and $t_1$  are not `close' to each other.
	
	\item[--] The  advantage of our attack over \cite{Ganju18,Zhang21, Chase21} is that we do not require the need to train an ensemble of shadow models for the $(t_0,t_1)$-distinguishability test. 
	
	\item[--] We perform experiments on the Adult dataset, where we evaluate our attacks on various subpopulations, created using feature matching,  and show that the adversay is able to succesfully distinguih if the dataset had $t_0$ or $t_1$ fraction of samples of the target property.
\end{itemize}
\end{comment}
